On simple expectations and observations of intelligent agents: A complexity study

Public observation logic (POL) reasons about agent expectations and agent observations in various real world situations. The expectations of agents take shape based on certain protocols about the world around and they remove those possible scenarios where their expectations and observations do not match. This in turn influences the epistemic reasoning of these agents. In this work, we study the computational complexity of the satisfaction problems of various fragments of POL. In the process, we also highlight the inevitable link that these fragments have with the well-studied Public announcement logic.

==> section_fullPOL.tex <==
    Before tackling the full POL language, let us discuss a small fragment of the single-letter fragment as a preliminary. That fragment $\mathcal L_1$ we consider contains the dynamic modalities $\ldiaarg a$ and $\ldiaarg {a^*}$. That fragment can be solved by reducing to epistemic linear-temporal-logic as follows. We consider the following translation:

\newcommand{\alive}{\textsf{alive}}

    \begin{align*}
        tr(p) & = p \\
        tr(\ldiaarg a \phi) & = X(\alive \land tr(\phi) \\
        tr(\ldiaarg {a^*} \phi) & = F(\alive \land tr(\phi) \\
        tr(K_i \phi) & = K_i(\alive \rightarrow tr(\phi)
    \end{align*}

    where $\alive$ is a fresh atomic propositions saying that the state is surviving.


\begin{proposition}
Let $\phi$ be a POL-formula in the fragment $\mathcal L_1$. Then $\phi$ is POL-sat iff $$tr(\phi) \land \alive \land G(\lnot \alive \rightarrow G\lnot \alive) \land \bigwedge_{p \in \phi} p \rightarrow Gp \land \lnot p \rightarrow G \lnot p$$ is LTLK-sat.
\end{proposition}

Some thoughts:
\begin{itemize}
    \item I guess. The "full single-letter fragment" can be captured in the same spirit. A bit more involved.. we have to capture each $|\pi]$ which may be equivalent to let $[a^*]\phi \lor [aaaa] \phi$... 
    \item If we have several letters in $\Sigma$, the time starts to be branching too. A comparison with epistemic CTL? But still it should be "deterministic" according a letter, which is difficult to encode in CTL. 
\end{itemize}

==> tableau-multi-word.tex <==
Here, in this section, we design a proof system using tableau method to prove satisfiability. But before that, let us introduce some inferences that are valid in $\POL$, and this will help in understanding tableau inferences we design. 
\subsection{Axioms}\label{axiomsect}
\begin{itemize}
    % \item The Perfect recall axiom is given by: $$
    % \ldiaarg{a}\hat{K}\varphi\rightarrow\hat{K}\ldiaarg{a}\varphi
    % $$. Informally, if after observing an atomic observation $a$, agent considers $\varphi$ a possibility, then it considers it possible that after observing $a$, $\varphi$ holds. From the point of view of Epistemic Expectation Model, for any world $s, t$ in model $\M$, if $s$ is in $\M|_a$ and $s\sim t$ in $\M|_a$, then $s\sim t$ in $\M$.
    
    % \item The No Miracle axiom is given by:
    % $$
    % \hat{K}\ldiaarg{a}\varphi\rightarrow [a]\hat{K}\varphi
    % $$
    % From the point of view of Epistemic Expectation Model, for any world $s, t$ in model $\M$, if $s\sim t$ in $\M$ and $s,t$ is in $\M|_a$, then $s\sim t$ in $\M|_a$.
    
    \item The constant Valuation axiom is given by:
    $$
    p\rightarrow [\pi]p
    $$, where $p$ is a propositional formula. This axiom interprets as after any observation, the propositional world remains same, that is, informally, after observation, the world in the residued model remains same according to propositional valuation, only residues its expectation.
    
    \item The determinism axiom is given by:
    $$
    \ldiaarg{a}\varphi\rightarrow [a]\varphi
    $$
    , where $a$ is an atomic observation. The axiom suggests that given an epistemic expectation model $\M$ and an atomic observation $a$, $\M|_a$ is unique.
\end{itemize}

 Each tableau term is of the form $(\sigma\ \ w\ \ \varphi)$ or $(\sigma\ \ w\ \ \checkmark)$ or $(\sigma_1,\sigma_2)_i$, where $w\in\Sigma^*$, $\varphi\in\POL_1$ and $\sigma, \sigma_1, \sigma_2$ are labels. 

Intuitively, each label represents a world in the model. 

The term $(\sigma\ \ w\ \ \varphi)$ represents the world representing $\sigma$ survives after projecting the model on $w$ and in that world $\varphi$ is satisfiable. 

The term $(\sigma\ \ w\ \ \checkmark)$ represents that the world represented by $\sigma$ survives under projection of $w$ of the model.

The term $(\sigma_1,\sigma_2)_i$ represents in the model, the worlds represented by $\sigma_1$ and $\sigma_2$ should be indistinguishable to the agent $i\in Agt$, where $Agt$ is finite set of agents.

Now we define the inference rules of our tableau proof system. Here an inference rule looks like:
\infer{C_1 | C_2 | \ldots | C_n}{%
                        A
                        }.

Here each $C_i$ and $A$ is a set of tableau terms. The $C_i$s are called consequence, $A$ is the antecedent.

A tableau proof can be assumed a tree. Each node of the tree is a set of tableau terms $\Gamma$. An inference rule can be applied in the following way:

If $A\subseteq\Gamma$ and $C_i$'s are not in $\Gamma$, the children of $\Gamma$ are $\Gamma\union C_i$ for each $i\in[n]$.

When no rules can be applied on a $\Gamma$, we say $\Gamma$ is saturated (leaf node in the proof tree).

If $\bot\in\Gamma$, we say that branch is closed. If all branch of the proof tree is closed, we say the tableau is closed, else is open.

Given a $\POL_1$ formula $\varphi$, we start with $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma,\sigma)_{i\in Agt}, (\sigma\ \ \epsilon\ \ \checkmark)\}$.

For space reasons, the term $(\sigma_1, \sigma_2)_{i\in Agt}$ interprets as the set of terms $\{(\sigma_1,\sigma_2)_i\mid i\in Agt\}$.

\subsection{Rules}
\begin{itemize}
    \item Propositional Rules
    \begin{itemize}
        \item Clash rule:
        \infer{\bot}{%
                        (\sigma
                        & w
                        & p),
                        & (\sigma
                        & w
                        & \neg p)
                        }, $p\in\mathcal{P}$
        \item Constant Valuation if:
        \infer{(\sigma\ \ w\ \ [a]p)}{%
                        (\sigma
                        & w
                        & p)
                        }, $p\in\mathcal{P}$, $a\in\Sigma$           
        \item Constant Valuation Negation if:
        \infer{(\sigma\ \ w\ \  [a]\neg p)}{%
                        (\sigma
                        & w
                        & \neg p)
                        }, $p\in\mathcal{P}$, $a\in\Sigma$

        \item AND rule:
        \infer{(\sigma\ \ w\ \ \psi),(\sigma\ \ w\ \  \chi)}{%
                        (\sigma
                        & w
                        & \psi\wedge\chi)
                        }

        \item OR rule:
        \infer{(\sigma\ \ w\ \ \psi)|(\sigma\ \ w\ \ \chi)}{%
                        (\sigma
                        & w
                        & \psi\vee\chi)
                        }

        
    \end{itemize}

    \item Knowledge Rules
    \begin{itemize}
        \item Knowledge: 
        \infer{(\sigma'\ \ w\ \ \psi)}{%
                        (\sigma
                        & w
                        & K_i\psi),
                        &(\sigma'
                        & w
                        & \checkmark),
                        &(\sigma, \sigma')_i
                        }, $i\in Agt$

        \item Possibility:
        \infer{(\sigma,\sigma_n)_i, (\sigma_n\ \ w\ \ \checkmark), (\sigma_n\ \ w\ \  \psi), (\sigma_n, \sigma_n)_{i\in Agt}}{%
                        (\sigma
                        & w
                        & \hat{K_i}\psi)
                        },
        \infer{(\sigma,\sigma')_i}{%
                        (\sigma, \sigma'')_i,
                        & (\sigma'',\sigma')_i
                        },
        \infer{(\sigma,\sigma')_i}{%
                        (\sigma', \sigma)_i
                        }, $i\in Agt$

        % \item No Miracle ? (\textbf{UNDECIDED}): 
        % \infer{\sigma\ \ [a]\hat{K}\psi\ \ w}{%
        %                 \sigma
        %                 & \hat{K}\langle a\rangle\psi
        %                 & w
        %                 }
    \end{itemize}

    \item Diamond and Box Rules:
    \begin{itemize}
        \item Diamond Decompose:
        \infer{(\sigma\ \ w\ \ \langle a\rangle\langle w'\rangle\psi)}{%
                        (\sigma
                        & w
                        & \langle aw'\rangle\psi)
                        }

        \item Box Decompose:
        \infer{(\sigma\ \ w\ \ [a][w']\psi)}{%
                        (\sigma
                        & w
                        & [aw']\psi)
                        }
                        

        \item Diamond Project: 
        \infer{(\sigma\ \ wa\ \ \checkmark), (\sigma\ \ wa\ \ \psi)}{%
                        (\sigma
                        & w
                        & \langle a\rangle\psi)
                        }

        \item Box Project:
        \infer{(\sigma\ \ wa\ \ \psi)}{%
                        (\sigma
                        & w
                        & [a]\psi),
                        & (\sigma\ \ wa\ \ \checkmark)
                        }
                        
        \item Project Determinism:
        \infer{(\sigma\ \ w\ \ [a]\psi)}{%
                        (\sigma
                        & w
                        & \langle a\rangle\psi)
                        }
                        
        % \item Perfect Recall ? (\textbf{UNDECIDED}):
        % \infer{\sigma\ \ \hat{K}\langle a\rangle\psi\ \ w}{%
        %                 \sigma
        %                 & \langle a\rangle\hat{K}\psi
        %                 & w
        %                 }
    \end{itemize}
    
    \item Survival Rules:
    \begin{itemize}
        \item Constant Valuation Up:
        \infer{(\sigma\ \ \epsilon\ \ p)}{%
                        (\sigma
                        & w
                        & p)
                        },
        \infer{(\sigma\ \ \epsilon\ \ \neg p)}{%
                        (\sigma
                        & w
                        & \neg p)
                        }, $p\in\mathcal{P}$
                        
        \item Survival Chain:
        \infer{(\sigma\ \ w\ \ \checkmark)}{%
                        (\sigma
                        & wa
                        & \checkmark)
                        }, $a\in\Sigma, w\in\Sigma^*$
    \end{itemize}
\end{itemize}

% \subsubsection{Proof that PR and NM Axiom Valid in $\POL_1$}
% Here we prove two axioms, Perfect Recall ($\ldiaarg{a}\hat{K}\psi\rightarrow\hat{K}\ldiaarg{a}\psi$) and No Miracle($\hat{K}\ldiaarg{a}\psi\rightarrow[a]\hat{K}\psi$), to be valid in $\POL_1$.
% \begin{theorem}
% For any $\POL_1$ formula $\psi$, and any $\POL$ model $\M = \ldiaarg{W, R, V, Exp}$, $\M,s\vDash\ldiaarg{a}\hat{K}\psi\rightarrow\hat{K}\ldiaarg{a}\psi$.\label{theorem:PRvalidity}
% \end{theorem}
% \begin{proof}
% Let us assume $\M,s\vDash\ldiaarg{a}\hat{K}\psi$.
% \begin{align*}
%     &\M,s\vDash\ldiaarg{a}\hat{K}\psi\\
%     &\implies \M|_a,s\vDash\hat{K}\psi\\
%     &\implies\exists(s,t)\in R_a\subseteq R\mbox{ and }\M|_a,t\vDash\psi\mbox{, where $R_a$ is the relation set of $\M|_a$}\\
%     &\implies\M,t\vDash\ldiaarg{a}\psi\\
%     &\implies\M,s\vDash\hat{K}\ldiaarg{a}\psi\mbox{, since $R_a\subseteq R$}
% \end{align*}
% \end{proof}
% Next we prove validity of NM.
% \begin{theorem}
% For any $\POL_1$ formula $\psi$, and any $\POL$ model $\M = \ldiaarg{W, R, V, Exp}$, $\M,s\vDash\hat{K}\ldiaarg{a}\psi\rightarrow[a]\hat{K}\psi$.\label{theorem:NMvalidity}
% \end{theorem}
% \begin{proof}
% Let us assume $\M,s\vDash\hat{K}\ldiaarg{a}\psi$.
% \begin{align*}
%     &\M,s\vDash\hat{K}\ldiaarg{a}\psi\\
%     &\implies\exists(s,t)\in R\mbox{ and }\M,t\vDash\ldiaarg{a}\psi\\
%     &\implies\M|_a,t\vDash\psi
% \end{align*}
% Now let us assume $s\notin W_a$ where $W_a$ is the set of worlds in $\M|_a$. Then vacuously, $\M,s\vDash[a]\hat{K}\psi$.

% Now suppose $s\in W_a$. Hence $(s,t)\in R_a$, where $R_a\subseteq R$ is the set of indistinguishability relation of $\M|_a$. Therefore $\M|_a,s\vDash\hat{K}\psi$. This implies $\M,s\vDash[a]\hat{K}\psi$.
% \end{proof}

\subsubsection{Termination}
Before proving termination, let us define an important notion of Fischer Ladner Closure of a formula.
\begin{defi}
\textbf{Fischer-Ladner Closure} The Fisher-Ladner closure of a formula $\varphi$ , denoted $FL(\varphi)$, is the minimal set satisfying
    \begin{itemize}
        \item $\varphi\in FL(\varphi)$
        \item if $\psi\in FL(\varphi)$ then $\neg\psi \in FL(\varphi)$, provided $\psi$ does not start with $\neg$
        \item if $\neg\psi, \psi\wedge\chi, K_i\psi$ or $[\pi]\psi$ are in $FL(\varphi)$ then $\psi,\chi \in FL(\varphi)$
        \item if $[\pi_1;\pi_2]\psi \in FL(\varphi)$ then $[\pi_1][\pi_2]\psi \in FL(\varphi)$
        \item if $[\pi_1+\pi_2]\psi \in FL(\varphi)$ then both $[\pi_1]\psi$ and $[\pi_2]\psi$ are in $FL(\varphi)$
        \item if $[\pi^{\star}]\psi \in FL(\varphi)$ then $[\pi][\pi^\star]\psi \in FL(\varphi)$
    \end{itemize}
\end{defi}
\begin{theorem}
Given the formula $\varphi$, the tableau proof for satisfiability terminates.
\label{lemma:terminationwordmulti}
\end{theorem}
\begin{proof}
We can prove that a term like $(\sigma\ \ w\ \ \varphi)$, for any $w$ and any $\sigma$, the tableau proof for $\{(\sigma\ \ w\ \ \varphi), (\sigma,\sigma)_{i\in Agt}, (\sigma\ \ w\ \ \checkmark)\}$ terminates, by induction on the size of $\varphi$.

\textbf{Base Case.} Consider the case where $\varphi = p$ where $p$ is a propositional letter. Starting from $\Gamma = \{(\sigma\ \ w\ \ \varphi), (\sigma,\sigma)_{i\in Agt}, (\sigma\ \ \epsilon\ \ w)\}$, the tableau applies constant valuation rule $|\Sigma|$ times and then the tableau terminates here since no more rule can be applied.

\textbf{Induction Hypothesis.} Let the statement be true any $\varphi$ such that $|\varphi| = n$.

\textbf{Induction Step.} Consider $\varphi$ such that $|\varphi| = n + 1$. We go case by case in syntax of $\varphi$:
\begin{itemize}
    \item $\varphi = \psi\wedge\chi$. Here, the AND rule gets applied to produce $(\sigma\ \ w\ \ \psi)$ and $(\sigma\ \ w\ \ \chi)$, and by IH proof for them terminates.
    
    \item $\varphi = \psi\vee\chi$. Here the OR rule will give $(\sigma\ \ w\ \ \psi)$ or $(\sigma\ \ w\ \ \chi)$ which again is terminating.
    
    \item $\varphi = K_i\psi$. By the knowledge rule , the term $(\sigma' \ \ w\ \ \psi)$ gets added for every terms as $(\sigma, \sigma')_i$ and $(\sigma'\ \ w\ \ \checkmark)$. By IH, this terminates.
    
    \item $\varphi = \hat{K_i}\psi$. By the possibility rule, we introduce a new label $\sigma_n$ and term $(\sigma_n\ \ w\ \ \psi)$ as well as the relational terms and the survival terms $(\sigma_n\ \ w\ \ \checkmark)$. The Survival Chain rule hence adds $|w|$ many checkmark terms. Also, since by IH, number of unique previously produced world labels are finite, say $l$, hence the relational terms for $\sigma_n$ adds at most $l\times |Agt|$ more relation terms. By IH, proof for this terminates.
    
    \item $\varphi = \ldiaarg{a\pi}\psi$. By the diamond decompose we derive $(\sigma\ \ w\ \ \ldiaarg{a}\ldiaarg{\pi}\psi)$ and by diamond project, we derive $(\sigma\ \ wa\ \ \checkmark)$ and $(\sigma\ \ wa\ \ \psi)$. By IH, the proof for this terms terminate.
    
    \item $\varphi = [a\pi]\psi$. By box decompose, we derive $(\sigma\ \ w\ \ [a][\pi]\psi)$. If term $(\sigma\ \ wa\ \ \checkmark)$ already derived, by box project $(\sigma\ \ wa\ \ [\pi]\psi)$ is derived, and by IH, the proof for this term terminates.
\end{itemize}

Now for every $\hat{K}$, there arrives a new label $\sigma'$, and for every $\ldiaarg{a}$ operator, a letter gets added in $w$. Hence $\#\sigma = O(|\varphi|)$, where $\#\sigma$ is number of unique world labels. Also since max legnth of such a $w$ is at most $O(|\varphi|)$, because of survival chain, there can be $|w|$ many terms derived and hence polynomial to size of $|\varphi|$ such terms. Since there can be at most $\Sigma^{O(|\varphi|)}$ such unique words, hence the proof terminates, that is arrives at a point where it cannot derive more new terms.
\end{proof}


\subsubsection{Soundness and Completeness}
\begin{theorem}
Given a formula $\varphi$, if $\varphi$ is satisfiable, then the tableau for $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$ is open.
\end{theorem}

\begin{theorem}
Given a formula $\varphi$, if the tableau for $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$ is open, then $\varphi$ is satisfiable.
\end{theorem}
\begin{proof}
Since by assumption, the tableau for $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$ is open, there exists a branch in the tableau tree where in the leaf node there is  a set of terms $\Gamma_l$ such that it is saturated and $\bot\notin\Gamma_l$.

For the purpose of this proof, let us define a relation over the words $\bar{w}$ that appears in $\Gamma_l$. For any two word $\bar{w}_1$ and $\bar{w}_2$ that appears in $\Gamma_l$, $\bar{w}_1\leq_{pre}\bar{w}_2$ if and only if $\bar{w}_1\in\LL(Pre(\bar{w}_2))$. Now, this relation is reflexive ($\bar{w}_1\in\LL(Pre(\bar{w}_1))$), asymmetric (if $\bar{w}_1\in\LL(Pre(\bar{w}_2))$ and $\bar{w}_2\in\LL(Pre(\bar{w}_1))$ then $\bar{w}_1 = \bar{w}_2$) and transitive (if $\bar{w}_1\in\LL(Pre(\bar{w}_2))$ and $\bar{w}_2\in\LL(Pre(\bar{w}_3))$ then $\bar{w}_1\in\LL(Pre(\bar{w}_3))$). Hence this relation creates a partial order among all the words occuring in $\Gamma_l$. We also denote $\bar{w_1}<_{pre}\bar{w_2}$ to interpret the fact that $\bar{w_1}\leq_{pre}\bar{w_2}$ and $\bar{w_1}\neq\bar{w_2}$.

Now we create a model $\M = \ldiaarg{W, R, V, Exp}$ out of $\Gamma_l$ and prove that $\varphi$ is satisfied by some world in the model.

\begin{itemize}
    \item $W = \{s_\sigma\mid \sigma\mbox{ is a distinct label in the terms occuring in }\Gamma_l\}$
    
    \item $R = \{\{s_{\sigma_1}, s_{\sigma_2}\}\mid(\sigma_1,\sigma_2)\in\Gamma_l\}$
    
    \item $V(s_\sigma) = \{p\mid (\sigma\ \ \epsilon\ \ p)\in\Gamma_l\}$
    
    \item $Exp(s_\sigma) = \sum_{w\in\Lambda_\sigma}w$, where $\Lambda_\sigma = \{w\mid (\sigma\ \ w\ \ \checkmark)\in\Gamma_l\mbox{ and }\nexists w':((\sigma\ \ w'\ \ \checkmark)\in\Gamma_l\mbox{ and }w<_{pre} w')\}$
\end{itemize}

Note that, new world label $\sigma_n$ is only created in the possibility rule, with a reflexive relation on itself. Now consider the set $R' = \{(\sigma, \sigma')\mid \{(sigma\ \ w\ \ \checkmark), (\sigma' \ \ w'\ \ \checkmark)\}\subseteq\Gamma_l\}$. Hence this can be considered a binary relation over the set of all distinct $\sigma$ that occurs in $\Gamma_l$. When a $\sigma'$ is created by possibility rule, it is refexive. Also by the relation rules in possibility rule, they are made symmetrically related with every other label that has been previously there. Hence $R'$ is an equivalence relation, hence making $R$ in the model an equivalence relation.


Now we shall prove the following two statement:

\textbf{If $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$ then $s_{\sigma}$ survives in $\M|_w$}

and 

\textbf{If $(\sigma\ \ w\ \ \varphi)\in\Gamma_l$ and $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$ then $s_{\sigma}$ survives in $\M|_w$ and  $\M|_w,s_\sigma\vDash\varphi$}.


For the first statement, we induct on the size of $|w|$.

\textbf{Base Case.} Let $|w| = 1$. Hence $w \in \{\epsilon\}\union \Sigma$ . Since $\Gamma\subseteq\Gamma_l$ and $(\sigma\ \ \epsilon\ \ \checkmark)$, and $s_\sigma$ is in $\M|_\epsilon = \M$.

For the case $w = a$ for any $a\in\Sigma$. Hence there exists a word $w'$ that occurs in a term in $\Gamma_l$ labelled by $\sigma$ such that $w\in\LL(Pre(w'))$ and there is no other word bigger than $w'$ such that $w'$ is in its prefix, since by lemma \ref{lemma:terminationwordone}, the proof terminates. Hence by definition of $w'\in\LL(Exp(s_\sigma))$ which guarantees survival of $s_\sigma$ in $\M|_a$. 

\textbf{Induction Hypothesis.} Assume the statement to be true for $|w| = n$.

\textbf{Inductive Step.} Consider the case where $|w| = n + 1$. 

By assumption, $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$. Hence by the fact that $\Gamma_l$ is saturation and by rule "Survival Chain", there is $(\sigma\ \ w'\ \ \checkmark)\in\Gamma_l$, where $w = w'a$ for some $a\in\Sigma$. Hence by IH, the result follows that $s_\sigma$ survives in $\M|_{w'}$. 

Now, by termination, there are finite many unique words occuring in $\Gamma_l$. Clearly, $w'\leq_{pre} w$. Since there are finite many words, there is a $w_*$, which is of maximum size such that $w\leq_{pre} w_*$ and $(\sigma\ \ w_*\ \ \checkmark)\in\Gamma_l$. Hence $w_*\in\Lambda_\sigma$ in the definition of Exp of model. Therefore $w_*\in\LL(Exp(s_\sigma))$ and since $w'\leq_{pre} w\leq_{pre} w_*$, $s_\sigma$ survives in $\M|_{w'}$, hence $s_\sigma$ shall survive in $\M|_{w}$.

% Now, since $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$, there is a $w''$ occurring in a term of form $(\sigma\ \ w''\ \ \checkmark)\in\Gamma_l$  such that $w\in \LL(Pre(w''))$ and there is no $w'''$ such that $(\sigma\ \ w'''\ \ \checkmark)\in\Gamma_l$ and $w''\in\LL(Pre(w'''))$. Hence, by definition of the model ($Exp$), $w''\in\Lambda$, which further suggests $w''\in\LL(Exp(s_\sigma))$. Since $w\in\LL(Pre(w''))$ and $s_\sigma$ is in $\M|_{w'}$, therefore $s_\sigma$ survives in $\M|_{w}$. This proves the first part of the proof that if $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$, then $s_\sigma$ survives in $\M|_w$.

\textbf{Proof for Second Statement.}
Naturally, we shall induct upon the size of $w$ and $\varphi$. But the induction is such that the we assume hypothesis for larger $w$ and smaller $\varphi$, and we prove statement for smaller $w$ and larger $\varphi$. That is, let the statement be $\mathcal{P}(m, n)$, where $m = |w|$ and $n = |\varphi|$, assuming this we try proving $\mathcal{P}(m',n')$, where $m'\leq m$ and $n\geq n'$.

\textbf{Base Case.} Let $|w| = m$, where $m$ is maximum among all the size of words occurring in the terms of $\Gamma_l$. Therefore, $\varphi$ is not of the form $\ldiaarg{w}\psi$, where $w$ is a word over $\Sigma$, as $\Gamma_l$ is saturated. We prove it step by step on syntax of $\varphi$.
\begin{itemize}
    \item (Base Case for $\varphi$ in $m$), $\varphi = p$. Since $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$ hence $s_\sigma$ survives in $\M|_w$. Also, by constant valuation up, $(\sigma\ \ \epsilon\ \ p)\in\Gamma_l$. Hence By definition of model, $\M|_w,s_{\sigma}\vDash p$. Similar for negation.
    
    \item $\varphi = \hat{K}\psi$. Since $\Gamma_l$ is saturated, by the rule of possibility, $\{(\sigma'\ \ w\ \ \psi), (\sigma, \sigma'), (\sigma'\ \ w\ \ \checkmark)\}\subseteq\Gamma_l$. By IH on the subformula of $\varphi$, definition of model, the proof of previous statement, and the rule "survival chain", $s_{\sigma'}$ survives in $\M|_{w}$ and $\M|_w,s_{\sigma'}\vDash\psi$. Also by definition, $\{s_{\sigma}, s_{\sigma'}\}\in R$, hence proving $\M|_w, s_\sigma\vDash\hat{K}\psi$.
    
    \item $\varphi = K\psi$. Since $\Gamma_l$ is saturated, and by previous statement $s_{\sigma'}$ is surviving for every $(\sigma'\ \ w\ \ \checkmark)$, by the rule of knowledge $(\sigma'\ \ w\ \ \psi)\in\Gamma_l$ for every $(\sigma, \sigma')$. Hence by IH on subformula, $\M|_w, s_{\sigma'}\vDash\psi.$
    
    \item $\varphi = [w']\psi$. Since $m$ is the biggest, there is no $(\sigma\ \ wa\ \ \checkmark)\in\Gamma_l$ and hence vacuously, $\M|_w,s_\sigma\vDash[a]\psi$.
    
\end{itemize}

\textbf{Induction Hypothesis.} Let us consider the statement is true for any $w$ and $\varphi$ such that $|w|>m'$ and $|\varphi|<n'$ for some $m'$ and $n'$.

\textbf{Inductive Step.} We prove for $|w| = m'$ and $|\varphi| = n'$. Again, we go case by case on syntax of $\varphi$. The cases proof for every syntax other than $\ldiaarg{a}\psi$ is same as previous.

Hence let $\varphi = \ldiaarg{a}\psi$. Since $\Gamma_l$ is saturated, $\{(\sigma\ \ wa\ \ \checkmark), (\sigma\ \ wa\ \ \psi)\}\subseteq\Gamma_l$ by the diamond rule. By the proof of the previous statement, $s_\sigma$ survives in $\M|_{wa}$. Also by IH on $|w|$ as well as $|\varphi|$, $\M|_{wa},s_\sigma\vDash\psi$. Hence, $\M|_w,s_\sigma\vDash\ldiaarg{a}\psi$.

Similar proof goes for box.
\end{proof}

\subsubsection{A $\PSPACE$ upper bound}
In this section, we design an algorithm based on tableau and prove existence of an algorithm that takes polynomial space with respect to the size of $\varphi$. Now given a $\varphi$, we now create a tree of nodes that contains terms of the form $(w, \psi)$ and $(w, \checkmark)$, where $w\in \Sigma^*$ is a word that is occuring in tableau, and $\psi$ is a formula in $FL(\varphi)$. Each node $T_\sigma$ refers to a world label $\sigma$ in tableau, a term of the $(w,\psi)\in T_\sigma$ intuitively translates to in the world corresponding to $\sigma$, after projecting model on $w$, the world survives and there $\psi$ is satisfied. Similarly, $(w, \checkmark)\in T_\sigma$ means world corresponding to $\sigma$ survives after projection on $w$. 

For this algorithm, we change the definition of saturation and unsaturation a bit from the earlier definition. We say $T_\sigma$ is \textbf{unsaturated} against a rule $R$ iff there is a term in $(w, \psi)\in T_\sigma$ or $(w, \checkmark)\in T_\sigma$, such that $(\sigma\ \ w\ \ \psi)$ or $(\sigma\ \ w\ \ \checkmark)$ lies in the numerator of $R$ but there is no denominator $(\sigma\ \ w\ \ \psi')$ of $R$ such that $(w, \psi')$ is in $T_\sigma$, similar for terms like $(w, \checkmark)$. We call the term $(w, \psi)$ or $(w, \checkmark)$ here to be the \textbf{reason for unsaturation}.

Now, given $\varphi$, we start with the set of terms $T_{\sigma_0} = \{(\epsilon, \varphi), (\epsilon, \checkmark)\}$.
\begin{itemize}
    \item Start with $T_{\sigma_0}$ as the root of tree $\cT_P$.

    \item If there is a leaf node $T_\sigma$ of $\cT_P$ as long as the conditions from (1) - (4) satisfy:
    \begin{enumerate}
        \item If $\bot\notin T_\sigma$ and $T_\sigma$ is unsaturated against Propositional and Survival Rules then
        \begin{enumerate}
            \item Let $(w, \psi)$ or $(w, \checkmark)$ be the reason for unsaturation against the above rules.

            \item If $\psi = \psi_1\wedge\psi_2$, then $T_\sigma = T_\sigma\union\{(w, \psi_1),(w, \psi_2)\}$

            \item If $\psi = \psi_1\vee\psi_2$, then non deterministically choose $\psi_1$ or $\psi_2$ and $T_{\sigma} = T_\sigma\union\{(w, \psi_1)\}$ or $T_{\sigma} = T_\sigma\union\{(w, \psi_2)\}$ as per choice.

            \item If $\psi = l$ where $l$ is a literal then $T_\sigma = T_\sigma\union\{(w, [a]l), (\epsilon, l)\}$.

            \item If $\{(w, \psi), (w, \neg\psi)\}\subseteq T_\sigma$ the $T_\sigma = T_\sigma\union\{\bot\}$.

            \item If $(w, \checkmark)\in T_\sigma$ then $T_\sigma = T_\sigma\union\{(w',\checkmark)\mid w'\in Pre(\LL(w))\}$.
        \end{enumerate}

        \item If $\bot\notin T_\sigma$ and $T_\sigma$ is propositionally saturated but unsaturated against Box and Diamond Rules then
        \begin{enumerate}
            \item Let the reason for unsaturation be $(w, \psi)$.

            \item If $\psi = [w_1w_2]\psi'$ then $T_\sigma = T_\sigma\union\{(w, [w_1][w_2]\psi')\}$.

            \item If $\psi = \ldiaarg{w_1w_2}\psi'$ then $T_\sigma = T_\sigma\union\{(w,\ldiaarg{w_1}\ldiaarg{w_2}\psi')\}$.

            \item If $\psi = \ldiaarg{a}\psi'$ then $T_\sigma = T_\sigma\union\{(wa, \checkmark), (wa, \psi'), (w, [a]\psi')\}$.

            \item If $\psi = [a]\psi'$ and $(wa,\checkmark)\in T_\sigma$ then $T_\sigma = T_\sigma\union\{(wa, \psi')\}$
        \end{enumerate}

        \item If $\bot\notin T_\sigma$ and it saturated against Propositional, Survival and Box, Diamond Rules but for all formula $\psi$ that occurs in terms $(w, \psi)\in T_\sigma$, there is a $\psi'\in FL(\psi)$ such that neither $\psi'$ nor $\neg\psi'$ occurs in $T_\sigma$ then
        \begin{enumerate}
            \item Non-deterministically choose $\psi'$ or $\neg\psi'$ and $T_\sigma = T_\sigma\union\{(w,\psi')\}$ or $T_\sigma = T_\sigma\union\{(w,\neg\psi')\}$ as per choice, where $\neg\psi'$ is in Negation normal form.
        \end{enumerate}

        \item If $\bot\notin T_\sigma$ and $T_\sigma$ is saturated against Propositional rules, Survival Rules and Diamond, Box rules and there is no formula $\psi$ that occurs as $(w, \psi)\in T_\sigma$, there is a $\psi'\in FL(\psi)$ such that neither $\psi'$ nor $\neg\psi'$ occurs in $T_\sigma$ then
        \begin{enumerate}
            \item For every $(w, \hat{K_i}\psi)\in T_\sigma$ do
            \begin{itemize}
                \item $T = \{(w, \hat{K_i}\psi')\mid (w, \hat{K_i}\psi')\in T_\sigma\}\union \{(w, K_i\psi')\mid (w, K_i\psi')\in T_\sigma\}\union\{(w, \psi)\}$
                \item If there is no $i$-ancestor $T_{\sigma''}$ of $T_\sigma$ such that $T\subseteq T_{\sigma''}$ then add a $i$-child $T_{\sigma'} = T$
            \end{itemize}
        \end{enumerate}
    \end{enumerate}

    \item Mark nodes of $\cT_P$ as following:
    \begin{enumerate}
        \item If a leaf $T_\sigma$ has $\bot$ in it or $\{(w, K_i\psi), (w, \neg\psi)\}\subseteq T_\sigma$, mark it "UNSAT"

        \item A node $T_\sigma$ is marked "SAT" if all its children is marked "SAT" and $\{(w, K_i\psi), (w, \neg\psi)\}\nsubseteq T_\sigma$ 
    \end{enumerate}

    \item If $T_{\sigma_0}$ is marked "SAT" return SAT else UNSAT.
\end{itemize}

\paragraph{Corrctness} Now we reason that indeed if $\varphi$ is satisfiable the root node is marked SAT, else it is marked UNSAT.
\begin{theorem}
    Given $\varphi$, if it is satisfiable then the root node of the $cT_P$ is marked SAT.
\end{theorem}
\begin{proof}
    We prove this on induction on $m = depth(\cT_P) + |T_{\sigma_0}|$. 
    
    \textbf{Base Case}. Let $m = 2$ hence $\cT_P$ has only one node that is the root of size $2$. Hence $\varphi = l$ where $l$ is a literal or $\varphi = [a]\psi$. This makes the statement trivially true.

    \textbf{Induction Hypothesis}. Let the statement be true for every $m\leq k$.

    \textbf{Inductive Step}. Let $m = k+1$. Now we go case by case of $\varphi$:
    \begin{itemize}
        \item $\varphi = \psi_1\wedge\psi_2$. Since $\varphi$ is satisfiable, and if $\M,s\vDash\varphi$, hence $\M,s\vDash\psi_1$ and $\M,s\vDash\psi_2$. By IH, the $cT_p$ starting from $T_{\sigma_0} = \{(\epsilon, \psi_1), (\epsilon, \psi_2), (\epsilon, \checkmark)\}$, the root node will be marked SAT.

        \item $\varphi = \psi_1\vee\psi_2$. Since $\M,s\vDash\psi_1\vee\psi_2$, hence $\M,s\vDash\psi_1$ or $\M,s\vDash\psi_2$, assume the former. The algorithm nondeterministically will choose either $\psi_1$. By IH, starting from $T_{\sigma_0} = \{(\epsilon, \psi_1), (\epsilon, \checkmark)\}$, the root node will be marked SAT.

        \item $\varphi = \ldiaarg{a}\psi$. Since this this satisfiable, hence $\M,s\vDash\ldiaarg{a}\psi$ which implies $s\in\M|_a$ and $\M|_a, s\vDash\psi$, which also implies $\M,s \vDash [a]\psi$. By IH, starting from $T'_{\sigma_0} = \{(\epsilon, [a]\psi), (\epsilon, \checkmark), (a, \psi), (a, \checkmark)\}$, the root node gets marked SAT. The algorithm include $T'_{\sigma_0}$ in enumeration 2d.

        \item $\varphi = [a]\psi$. Assuming $\M,s\vDash [a]\psi$, the $s$ either survives or does not. The case of not survival is similar to in the base case. Say the $s$ is surviving in $\M$, by the case of diamond, $(a, \checkmark)\in T_{\sigma}$ and therefore the statement follows as in diamond case.

        \item $\varphi = \hat{K_i}\psi$. Since $\M,s\vDash\hat{K_i}\psi$ hence there is a $t\sim_i s$ where $\M,t\vDash\psi$, also $\M,t\vDash\hat{K_i}\psi'$ as well as $\M,t\vDash K_i\psi''$ for every $\{\hat{K_i}\psi', K_i\psi''\}\subseteq FL(\varphi)$ such that they are satisfied in $s$ . Consider the set $Epi(T) = \{(\epsilon, K_i\psi'')\mid (\epsilon, K_i\psi'')\in T_{\sigma}\}\union \{(\epsilon, \hat{K_i}\psi')\mid (\epsilon, \hat{K_i})\psi'\in T_{\sigma}\}$. By IH, $T\subseteq T_{\sigma_0}$ and also starting from $\{(\epsilon, \psi)\}\union T$, the root will be marked SAT. Since this is for any general $i$ and $\hat{K_i}\psi$, by IH, every $i-successor$ of $T_{\sigma_0}$ will be marked SAT and hence $T_{\sigma_0}$ is marked SAT, since the algorithm makes sure there is such an $i$ successor in step 4a.

        \item The proof goes similarly for $K_i$.
    \end{itemize}
\end{proof}

\begin{theorem}
    Given $\varphi$, If the root node is marked SAT then $\varphi$ is satisfiable.
\end{theorem}
\begin{proof}
    We create the model satisfying $\varphi$ using a similar method we used in correctness of tableau. 

    For the purpose of this proof, let us define a relation over the words $\bar{w}$ that appears in nodes $T_\sigma$. For any two word $\bar{w}_1$ and $\bar{w}_2$ that appears in $T_\sigma$, $\bar{w}_1\leq_{pre}\bar{w}_2$ if and only if $\bar{w}_1\in\LL(Pre(\bar{w}_2))$. Now, this relation is reflexive ($\bar{w}_1\in\LL(Pre(\bar{w}_1))$), asymmetric (if $\bar{w}_1\in\LL(Pre(\bar{w}_2))$ and $\bar{w}_2\in\LL(Pre(\bar{w}_1))$ then $\bar{w}_1 = \bar{w}_2$) and transitive (if $\bar{w}_1\in\LL(Pre(\bar{w}_2))$ and $\bar{w}_2\in\LL(Pre(\bar{w}_3))$ then $\bar{w}_1\in\LL(Pre(\bar{w}_3))$). Hence this relation creates a partial order among all the words occuring in $T_\sigma$. We also denote $\bar{w_1}<_{pre}\bar{w_2}$ to interpret the fact that $\bar{w_1}\leq_{pre}\bar{w_2}$ and $\bar{w_1}\neq\bar{w_2}$.

Now we create a model $\M = \ldiaarg{W, R, V, Exp}$ out of $\cT_P$ and prove that $\varphi$ is satisfied by some world in the model.

\begin{itemize}
    \item $W = \{s_\sigma\mid T_\sigma\mbox{ is a distinct node in the nodes occuring in }\cT_P\}$
    
    \item $R_i = \{\{s_{\sigma_1}, s_{\sigma_2}\}\mid T_{\sigma_1}\mbox{ is the i successor of }T_{\sigma_2}\mbox{ or vice-versa}\}$
    
    \item $V(s_\sigma) = \{p\mid (\epsilon, p)\in T_\sigma\}$
    
    \item $Exp(s_\sigma) = \sum_{w\in\Lambda_\sigma}w$, where $\Lambda_\sigma = \{w\mid (w, \checkmark)\in T_\sigma\mbox{ and }\nexists w':((w',\checkmark)\in T_\sigma\mbox{ and }w<_{pre} w')\}$
\end{itemize}

Similarly as in completeness, we essentially prove two statements:


\textbf{If $(w, \checkmark)\in T_\sigma$ then $s_{\sigma}$ survives in $\M|_w$}

and 

\textbf{For any word $w\in\Sigma^*$ that occurs in $T_\sigma$, If $(w, \varphi)\in T_\sigma$ and $(w,\checkmark)\in T_\sigma$ then $s_{\sigma}$ survives in $\M|_w$ and  $\M|_w,s_\sigma\vDash\varphi$}.


For the first statement, we induct on the size of $|w|$.

\textbf{Base Case.} Let $|w| = 1$. Hence $w \in \{\epsilon\}\union \Sigma$ . Let $w = \epsilon$. We start from $(\epsilon, \checkmark)$ in the root, also for every new successor $T_\sigma'$, step 1f makes sure $(\epsilon, \checkmark)\in T_\sigma'$ and $\epsilon\in Pre(LL(w'))$ for any $w'$, hence $s_\sigma$ survives in $\M|_\epsilon$.

For the case $w = a$ for any $a\in\Sigma$. Hence there exists a word $w'$ that occurs in a term in $T_\sigma$ labelled by $\sigma$ such that $w\in\LL(Pre(w'))$ and there is no other word bigger than $w'$ such that $w'$ is in its prefix, since it terminates. Hence by definition of $w'\in\LL(Exp(s_\sigma))$ which guarantees survival of $s_\sigma$ in $\M|_a$. 

\textbf{Induction Hypothesis.} Assume the statement to be true for $|w| = n$.

\textbf{Inductive Step.} Consider the case where $|w| = n + 1$. 

By assumption, $(w,\checkmark)\in T_\sigma$. Hence by the fact that $T_\sigma$ is saturated against every rule except Knowledge and Possibility and by "Survival Chain", there is $(w',\checkmark)\in T_\sigma$, where $w = w'a$ for some $a\in\Sigma$. Hence by IH, the result follows that $s_\sigma$ survives in $\M|_{w'}$. 

Now, by termination, there are finite many unique words occuring in $T_\sigma$. Clearly, $w'\leq_{pre} w$. Since there are finite many words, there is a $w_*$, which is of maximum size such that $w\leq_{pre} w_*$ and $(w_*,\checkmark)\in T_\sigma$. Hence $w_*\in\Lambda_\sigma$ in the definition of Exp of model. Therefore $w_*\in\LL(Exp(s_\sigma))$ and since $w'\leq_{pre} w\leq_{pre} w_*$, $s_\sigma$ survives in $\M|_{w'}$, hence $s_\sigma$ shall survive in $\M|_{w}$.

% Now, since $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$, there is a $w''$ occurring in a term of form $(\sigma\ \ w''\ \ \checkmark)\in\Gamma_l$  such that $w\in \LL(Pre(w''))$ and there is no $w'''$ such that $(\sigma\ \ w'''\ \ \checkmark)\in\Gamma_l$ and $w''\in\LL(Pre(w'''))$. Hence, by definition of the model ($Exp$), $w''\in\Lambda$, which further suggests $w''\in\LL(Exp(s_\sigma))$. Since $w\in\LL(Pre(w''))$ and $s_\sigma$ is in $\M|_{w'}$, therefore $s_\sigma$ survives in $\M|_{w}$. This proves the first part of the proof that if $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$, then $s_\sigma$ survives in $\M|_w$.

% \textbf{Proof for Second Statement.}
% Naturally, we shall induct upon the size of $w$ and $\varphi$. But the induction is such that the we assume hypothesis for larger $w$ and smaller $\varphi$, and we prove statement for smaller $w$ and larger $\varphi$. That is, let the statement be $\mathcal{P}(m, n)$, where $m = |w|$ and $n = |\varphi|$, assuming this we try proving $\mathcal{P}(m',n')$, where $m'\leq m$ and $n\geq n'$.

% \textbf{Base Case.} Let $|w| = m$, where $m$ is maximum among all the size of words occurring in the terms of $T_\sigma$. Therefore, $\varphi$ is not of the form $\ldiaarg{w}\psi$, where $w$ is a word over $\Sigma$, as $\Gamma_l$ is saturated. We prove it step by step on syntax of $\varphi$.
% \begin{itemize}
%     \item (Base Case for $\varphi$ in $m$), $\varphi = p$. Since $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$ hence $s_\sigma$ survives in $\M|_w$. Also, by constant valuation up, $(\sigma\ \ \epsilon\ \ p)\in\Gamma_l$. Hence By definition of model, $\M|_w,s_{\sigma}\vDash p$. Similar for negation.
    
%     \item $\varphi = \hat{K}\psi$. Since $\Gamma_l$ is saturated, by the rule of possibility, $\{(\sigma'\ \ w\ \ \psi), (\sigma, \sigma'), (\sigma'\ \ w\ \ \checkmark)\}\subseteq\Gamma_l$. By IH on the subformula of $\varphi$, definition of model, the proof of previous statement, and the rule "survival chain", $s_{\sigma'}$ survives in $\M|_{w}$ and $\M|_w,s_{\sigma'}\vDash\psi$. Also by definition, $\{s_{\sigma}, s_{\sigma'}\}\in R$, hence proving $\M|_w, s_\sigma\vDash\hat{K}\psi$.
    
%     \item $\varphi = K\psi$. Since $\Gamma_l$ is saturated, and by previous statement $s_{\sigma'}$ is surviving for every $(\sigma'\ \ w\ \ \checkmark)$, by the rule of knowledge $(\sigma'\ \ w\ \ \psi)\in\Gamma_l$ for every $(\sigma, \sigma')$. Hence by IH on subformula, $\M|_w, s_{\sigma'}\vDash\psi.$
    
%     \item $\varphi = [w']\psi$. Since $m$ is the biggest, there is no $(\sigma\ \ wa\ \ \checkmark)\in\Gamma_l$ and hence vacuously, $\M|_w,s_\sigma\vDash[a]\psi$.
    
% \end{itemize}

% \textbf{Induction Hypothesis.} Let us consider the statement is true for any $w$ and $\varphi$ such that $|w|>m'$ and $|\varphi|<n'$ for some $m'$ and $n'$.

% \textbf{Inductive Step.} We prove for $|w| = m'$ and $|\varphi| = n'$. Again, we go case by case on syntax of $\varphi$. The cases proof for every syntax other than $\ldiaarg{a}\psi$ is same as previous.

% Hence let $\varphi = \ldiaarg{a}\psi$. Since $\Gamma_l$ is saturated, $\{(\sigma\ \ wa\ \ \checkmark), (\sigma\ \ wa\ \ \psi)\}\subseteq\Gamma_l$ by the diamond rule. By the proof of the previous statement, $s_\sigma$ survives in $\M|_{wa}$. Also by IH on $|w|$ as well as $|\varphi|$, $\M|_{wa},s_\sigma\vDash\psi$. Hence, $\M|_w,s_\sigma\vDash\ldiaarg{a}\psi$.

% Similar proof goes for box.

% \end{proof}

\textbf{Proof for Second Statement.}
Naturally, we shall induct upon the size of  $\varphi$. 

\textbf{Base Case.} Let $\varphi = l$ where $l$ is a literal. By step 1d, $(\epsilon, l)\in T_\sigma$, and by 2f $(\epsilon, \checkmark)\in T_\sigma$. By definition of evaluation function, and by previous statement, $s_\sigma\in\M|_w$ and $\M|_w,s_\sigma\vDash l$.

\textbf{Induction Hypothesis.} Let us consider the statement is true for any $\varphi$ such that $n\leq k$ for some integer $k$.

\textbf{Inductive Step.} We prove for $n = k+1$. Again, we go case by case on syntax of $\varphi$. We only go over knowledge, possibility, diamond and box cases.

\begin{itemize}
    \item $\varphi = \hat{K_i}\psi$. Since $(w, \hat{K_i}\psi)\in T_\sigma$, therefore there is a $i$ successor to $T_\sigma$, $T_{\sigma'}$ such that $(w,\psi)\in T_{\sigma'}$. By IH, $\M|_w,s_{\sigma'}\vDash\psi$. By construction, $s_{\sigma'}\sim_i s_{\sigma}$. Also, since $(w, \checkmark)\in T_{\sigma}\hat T_{\sigma'}$, they both survive in $\M|_w$. Hence $\M|_w, s_\sigma\vDash\hat{K_i}\psi$.

    \item $\varphi = K_i\psi$. Since $(w, K_i\psi)\in T_\sigma$, hence all the $i$ successor as well $i$ parent of $T_\sigma$ has $(w, K_i\psi)$ in them by step 4a. By step 3a, since $\psi\in FL(K_i\psi)$ and hence the term $(w, \psi)$ has been included (non-deterministically, for the case where $\neg\psi$ is included, they clash in marking step) in all the successor, parent as well as in $T_\sigma$ itself. By IH, $s_\sigma\in\M|_w$ and $\M|_w, s{\sigma}\vDash \psi$ as well as $s_{\sigma'}\in\M|_w$ and $\M|_w, s_{\sigma'}\vDash\psi$, where $T_{\sigma'}$ is a $i$ parent or $i$ successor of $T_\sigma$. By construction $s_{\sigma'}\sim_i s_{\sigma}$ for all such $s_{\sigma'}$, which implies $\M|_w, s_\sigma\vDash K_i\psi$.

    \item $\varphi = \ldiaarg{a}\psi$. Since $(w, \ldiaarg{a}\psi)\in T_\sigma$, hence by step 2d, $\{(wa, \psi), (wa, \checkmark)\}\subseteq T_\sigma$. By IH and previously proved statement, $s_\sigma\in\M|_{wa}$ and $\M|_{wa}, s_\sigma\vDash\psi$, hence $\M|_w, s_\sigma\vDash\ldiaarg{a}\psi$. The box proof goes in a similar way.
\end{itemize}
\end{proof}

\paragraph{Deciding SAT uses Polynomial Space}
Now we prove an existence of an algorithm using the above to prove our PSPACE upper bound.
\begin{theorem}
    Deciding satisfiability of $\varphi$ of word fragment of $\POL$ uses polynomial space with respect ot $|\varphi|$.
\end{theorem}
\begin{proof}
    Given the tree $\cT_P$ we create in the procedure, a node is marked satisfiable iff it does not have bot, negation of the knowledge is not true and all its succesors are satisfiable.

    

    We prove three things:
    \begin{enumerate}
        \item Each node is of polynomial size.
        \item Maximum children a node can have is polynomial.
        \item The height of the tree is polynomial.
    \end{enumerate}

    \paragraph{First Statement}. Let us consider the number of words $w$ possible. A unique word is created letter by letter from diamond formulas of $\varphi$. Hence number of such words $w$ such that there is no word $w'$ which contains $w$ as prefix is at most $|\varphi|$. Also size of such $w$ is at most $|\varphi|$. For each such $w$, there can be at most $n$ many prefixes, each of size at most $n$, where $n = |\varphi|$. Hence the number of unique words is at most $n^3$. Also the number of formulas is at most $|FL(\varphi)|\leq O(|\varphi|)$. Hence each node is of at most $O(n^4)$ size.

    \paragraph{Second Statement} From a node $T_\sigma$, a child is created for every unique pair of $w$ and a $\hat{K_i}$ formula in $T_\sigma$. Number of such pairs possible is, as proved before, $O(n^4)$.

    \paragraph{Third Statement}. For proving this, we use $md(\Gamma)$, given a set of formulas $\Gamma$, is the maximum modal depth over all formulas in $\Gamma$. Finally we define $F(T_\sigma)$ as the set of formulas occuring in the node $T_\sigma$. 

    Consider $T_\sigma$, the node $T^i_{\sigma'}$ is $i$- successor of $T_\sigma$ and $T^j_{\sigma''}$ be the $j$ successor of $T^i_{\sigma'}$ ($i\neq j$). Note that all the formulas in $F(T^j_{\sigma''})$ are from FL closure of all the $K_j$ and $\hat{K_j}$ formulas from $F(T^i_{\sigma'})$.

    Also all the formulas in $F(T^i_{\sigma'})$ are in the FL closure of the $K_i$ and $\hat{K_i}$ formulas occusring in $T_\sigma$. Hence $md(T^j_{\sigma''})\leq md(F(T^i_{\sigma'}))$. Therefore, there can be at most $O(|\varphi|^c)$ such agent alterations in one path of $\cT_P$ (not linear because there can be polynomial many words paired with each formula).

    Now let us consider how many consecutive $i$ succesors can happen in a path. Note that we create a new $i$ successor of a node such that the knowledge formulas as well as possibility formulas in the successor as well as parent node are equal. Hence a path containing consecutive $i$ successor will have the same knowledge and possibility formulas. The only thing differing is the $\psi$ formula in step 4a. Therefore number of such unique $(w,\psi)$ is the maximum number of consecutive $i$-successor nodes in the path, which again some polynomial of $|\varphi|$ (at most $|\varphi|$ many formulas and polynomial many words.).

    Therefore, the height of $\cT_P$ is polynomial with respect to the $|\varphi|$.
    % When a child is created for a $\hat{K_i}$ formula such as $(w, \hat{K_i}\psi)$, we copy every epistemic formula from parent node along with $\psi$. Hence there exists one formula in the child node with a strictly one less $\hat{K_i}$ operator. Therefore, the modal depth with respect to possibility operator decreases strictly at every level of the $cT_P$. Hence the depth is linear with respect to $|\varphi|$.
\end{proof}

==> tableau-word.tex <==
Here, in this section, we design a proof system using tableau method to prove satisfiability. But before that, let us introduce some inferences that are valid in $\POL$, and this will help in understanding tableau inferences we design. 
\subsection{Axioms}\label{axiomsect}
\begin{itemize}
    % \item The Perfect recall axiom is given by: $$
    % \ldiaarg{a}\hat{K}\varphi\rightarrow\hat{K}\ldiaarg{a}\varphi
    % $$. Informally, if after observing an atomic observation $a$, agent considers $\varphi$ a possibility, then it considers it possible that after observing $a$, $\varphi$ holds. From the point of view of Epistemic Expectation Model, for any world $s, t$ in model $\M$, if $s$ is in $\M|_a$ and $s\sim t$ in $\M|_a$, then $s\sim t$ in $\M$.
    
    % \item The No Miracle axiom is given by:
    % $$
    % \hat{K}\ldiaarg{a}\varphi\rightarrow [a]\hat{K}\varphi
    % $$
    % From the point of view of Epistemic Expectation Model, for any world $s, t$ in model $\M$, if $s\sim t$ in $\M$ and $s,t$ is in $\M|_a$, then $s\sim t$ in $\M|_a$.
    
    \item The constant Valuation axiom is given by:
    $$
    p\rightarrow [\pi]p
    $$, where $p$ is a propositional formula. This axiom interprets as after any observation, the propositional world remains same, that is, informally, after observation, the world in the residued model remains same according to propositional valuation, only residues its expectation.
    
    \item The determinism axiom is given by:
    $$
    \ldiaarg{a}\varphi\rightarrow [a]\varphi
    $$
    , where $a$ is an atomic observation. The axiom suggests that given an epistemic expectation model $\M$ and an atomic observation $a$, $\M|_a$ is unique.
\end{itemize}

 Each tableau term is of the form $(\sigma\ \ w\ \ \varphi)$ or $(\sigma\ \ w\ \ \checkmark)$ or $(\sigma_1,\sigma_2)$, where $w\in\Sigma^*$, $\varphi\in\POL_1$ and $\sigma, \sigma_1, \sigma_2$ are labels. 

Intuitively, each label represents a world in the model. 

The term $(\sigma\ \ w\ \ \varphi)$ represents the world representing $\sigma$ survives after projecting the model on $w$ and in that world $\varphi$ is satisfiable. 

The term $(\sigma\ \ w\ \ \checkmark)$ represents that the world represented by $\sigma$ survives under projection of $w$ of the model.

The term $(\sigma_1,\sigma_2)$ represents in the model, the worlds represented by $\sigma_1$ and $\sigma_2$ should be indistinguishable to the agent.

Now we define the inference rules of our tableau proof system. Here an inference rule looks like:
\infer{C_1 | C_2 | \ldots | C_n}{%
                        A
                        }.

Here each $C_i$ and $A$ is a set of tableau terms. The $C_i$s are called consequence, $A$ is the antecedent.

A tableau proof can be assumed a tree. Each node of the tree is a set of tableau terms $\Gamma$. An inference rule can be applied in the following way:

If $A\subseteq\Gamma$ and $C_i$'s are not in $\Gamma$, the children of $\Gamma$ are $\Gamma\union C_i$ for each $i\in[n]$.

When no rules can be applied on a $\Gamma$, we say $\Gamma$ is saturated (leaf node in the proof tree).

If $\bot\in\Gamma$, we say that branch is closed. If all branch of the proof tree is closed, we say the tableau is closed, else is open.

Given a $\POL_1$ formula $\varphi$, we start with $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma,\sigma), (\sigma\ \ \epsilon\ \ \checkmark)\}$.

\subsection{Rules}
\begin{itemize}
    \item Propositional Rules
    \begin{itemize}
        \item Clash rule:
        \infer{\bot}{%
                        (\sigma
                        & w
                        & p),
                        & (\sigma
                        & w
                        & \neg p)
                        }, $p\in\mathcal{P}$
        \item Constant Valuation if:
        \infer{(\sigma\ \ w\ \ [a]p)}{%
                        (\sigma
                        & w
                        & p)
                        }, $p\in\mathcal{P}$, $a\in\Sigma$           
        \item Constant Valuation Negation if:
        \infer{(\sigma\ \ w\ \  [a]\neg p)}{%
                        (\sigma
                        & w
                        & \neg p)
                        }, $p\in\mathcal{P}$, $a\in\Sigma$

        \item AND rule:
        \infer{(\sigma\ \ w\ \ \psi),(\sigma\ \ w\ \  \chi)}{%
                        (\sigma
                        & w
                        & \psi\wedge\chi)
                        }

        \item OR rule:
        \infer{(\sigma\ \ w\ \ \psi)|(\sigma\ \ w\ \ \chi)}{%
                        (\sigma
                        & w
                        & \psi\vee\chi)
                        }

        
    \end{itemize}

    \item Knowledge Rules
    \begin{itemize}
        \item Knowledge: 
        \infer{(\sigma'\ \ w\ \ \psi)}{%
                        (\sigma
                        & w
                        & K\psi),
                        &(\sigma'
                        & w
                        & \checkmark),
                        &(\sigma, \sigma')
                        }

        \item Possibility:
        \infer{(\sigma,\sigma_n), (\sigma_n\ \ w\ \ \checkmark), (\sigma_n\ \ w\ \  \psi), (\sigma_n, \sigma_n)}{%
                        (\sigma
                        & w
                        & \hat{K}\psi)
                        },
        \infer{(\sigma,\sigma')}{%
                        (\sigma, \sigma''),
                        & (\sigma'',\sigma')
                        },
        \infer{(\sigma,\sigma')}{%
                        (\sigma', \sigma)
                        }

        % \item No Miracle ? (\textbf{UNDECIDED}): 
        % \infer{\sigma\ \ [a]\hat{K}\psi\ \ w}{%
        %                 \sigma
        %                 & \hat{K}\langle a\rangle\psi
        %                 & w
        %                 }
    \end{itemize}

    \item Diamond and Box Rules:
    \begin{itemize}
        \item Diamond Decompose:
        \infer{(\sigma\ \ w\ \ \langle a\rangle\langle w'\rangle\psi)}{%
                        (\sigma
                        & w
                        & \langle aw'\rangle\psi)
                        }

        \item Box Decompose:
        \infer{(\sigma\ \ w\ \ [a][w']\psi)}{%
                        (\sigma
                        & w
                        & [aw']\psi)
                        }
                        

        \item Diamond Project: 
        \infer{(\sigma\ \ wa\ \ \checkmark), (\sigma\ \ wa\ \ \psi)}{%
                        (\sigma
                        & w
                        & \langle a\rangle\psi)
                        }

        \item Box Project:
        \infer{(\sigma\ \ wa\ \ \psi)}{%
                        (\sigma
                        & w
                        & [a]\psi),
                        & (\sigma\ \ wa\ \ \checkmark)
                        }
                        
        \item Project Determinism:
        \infer{(\sigma\ \ w\ \ [a]\psi)}{%
                        (\sigma
                        & w
                        & \langle a\rangle\psi)
                        }
                        
        % \item Perfect Recall ? (\textbf{UNDECIDED}):
        % \infer{\sigma\ \ \hat{K}\langle a\rangle\psi\ \ w}{%
        %                 \sigma
        %                 & \langle a\rangle\hat{K}\psi
        %                 & w
        %                 }
    \end{itemize}
    
    \item Survival Rules:
    \begin{itemize}
        \item Constant Valuation Up:
        \infer{(\sigma\ \ \epsilon\ \ p)}{%
                        (\sigma
                        & w
                        & p)
                        },
        \infer{(\sigma\ \ \epsilon\ \ \neg p)}{%
                        (\sigma
                        & w
                        & \neg p)
                        }, $p\in\mathcal{P}$
                        
        \item Survival Chain:
        \infer{(\sigma\ \ w\ \ \checkmark)}{%
                        (\sigma
                        & wa
                        & \checkmark)
                        }, $a\in\Sigma, w\in\Sigma^*$
    \end{itemize}
\end{itemize}

% \subsubsection{Proof that PR and NM Axiom Valid in $\POL_1$}
% Here we prove two axioms, Perfect Recall ($\ldiaarg{a}\hat{K}\psi\rightarrow\hat{K}\ldiaarg{a}\psi$) and No Miracle($\hat{K}\ldiaarg{a}\psi\rightarrow[a]\hat{K}\psi$), to be valid in $\POL_1$.
% \begin{theorem}
% For any $\POL_1$ formula $\psi$, and any $\POL$ model $\M = \ldiaarg{W, R, V, Exp}$, $\M,s\vDash\ldiaarg{a}\hat{K}\psi\rightarrow\hat{K}\ldiaarg{a}\psi$.\label{theorem:PRvalidity}
% \end{theorem}
% \begin{proof}
% Let us assume $\M,s\vDash\ldiaarg{a}\hat{K}\psi$.
% \begin{align*}
%     &\M,s\vDash\ldiaarg{a}\hat{K}\psi\\
%     &\implies \M|_a,s\vDash\hat{K}\psi\\
%     &\implies\exists(s,t)\in R_a\subseteq R\mbox{ and }\M|_a,t\vDash\psi\mbox{, where $R_a$ is the relation set of $\M|_a$}\\
%     &\implies\M,t\vDash\ldiaarg{a}\psi\\
%     &\implies\M,s\vDash\hat{K}\ldiaarg{a}\psi\mbox{, since $R_a\subseteq R$}
% \end{align*}
% \end{proof}
% Next we prove validity of NM.
% \begin{theorem}
% For any $\POL_1$ formula $\psi$, and any $\POL$ model $\M = \ldiaarg{W, R, V, Exp}$, $\M,s\vDash\hat{K}\ldiaarg{a}\psi\rightarrow[a]\hat{K}\psi$.\label{theorem:NMvalidity}
% \end{theorem}
% \begin{proof}
% Let us assume $\M,s\vDash\hat{K}\ldiaarg{a}\psi$.
% \begin{align*}
%     &\M,s\vDash\hat{K}\ldiaarg{a}\psi\\
%     &\implies\exists(s,t)\in R\mbox{ and }\M,t\vDash\ldiaarg{a}\psi\\
%     &\implies\M|_a,t\vDash\psi
% \end{align*}
% Now let us assume $s\notin W_a$ where $W_a$ is the set of worlds in $\M|_a$. Then vacuously, $\M,s\vDash[a]\hat{K}\psi$.

% Now suppose $s\in W_a$. Hence $(s,t)\in R_a$, where $R_a\subseteq R$ is the set of indistinguishability relation of $\M|_a$. Therefore $\M|_a,s\vDash\hat{K}\psi$. This implies $\M,s\vDash[a]\hat{K}\psi$.
% \end{proof}
\subsubsection{The Tableau Algorithm}
Consider the following algorithm which is an iterative one that applies the above mentioned rules in some order. Given a formula $\varphi$, it starts with the set of terms $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma, \sigma), (\sigma\ \ \epsilon\ \ \checkmark)\}$. Then it keeps on applying the rules and adding terms, creating a tree of set of tableau terms.

% \begin{algorithm}[H]
% \caption{$\wordSATONE$}
% % \begin{algorithmic}
% % \SetAlgoLined
% % \caption{$\wordSATONE$}
% % \Require a formula $\varphi$
% % \Ensure Returns "SAT" if there exists a model satisfying $\varphi$, "UNSAT" otherwise
% $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$\\
% $\mathcal{T}$ be a tree of set of terms of tableau with $\Gamma$ in the root.\\
% \While{there is a case below applicable}{
%     \If{ there is a leaf in $\mathcal{T}$ that has no $\bot$ term and it is not saturated against Propositional and Survival Rules}{
%         Let $\Gamma$ be the leaf.\\
%         Let $(\sigma\ \ w\ \ \psi)$ or $(\sigma\ \ w\ \ \checkmark)$ be the term that are unsaturated.\\
%         $\Gamma' = \Gamma$\\
%         \If{$\psi = l$ where $l$ is of the form either $p$ or $\neg p$, where $p$ is a propositional letter}{
%             $\Gamma' = \Gamma'\union \{(\sigma\ \ w\ \ [a]\psi), (\sigma\ \ \epsilon\ \ \psi)\}$, by Constant valuation if and Up\\
%             Add $\Gamma'$ as a child of $\Gamma$.
%         }
%         \ElseIf{$\psi = \psi_1\wedge\psi_2$ }{
%             $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ \psi_1), (\sigma\ \ w\ \ \psi_2)\}$\\
%             Add $\Gamma'$ as a child of $\Gamma$.
%         }
%         \ElseIf{$\psi = \psi_1\vee\psi_2$}{
%             $\Gamma'_1 = \Gamma'\union\{(\sigma\ \ w\ \ \psi_1)\}$\\
%             $\Gamma'_2 = \Gamma'\union\{(\sigma\ \ w\ \ \psi_2)\}$\\
%             Add $\Gamma'_1$ and $\Gamma'_2$ as children of $\Gamma$
%         }
%         \ElseIf{$\{(\sigma\ \ w\ \ \psi), (\sigma\ \ w\ \ \neg\psi)\}\subseteq\Gamma$}{
%             $\Gamma' = \Gamma'\union\{\bot\}$\\
%             Add $\Gamma'$ as a child of $\Gamma$.
%         }
%         \Else{
%             $\Gamma' = \Gamma'\union\{(\sigma\ \ w'\ \ \checkmark)\mid w'\in Pre(\LL(w))\}$\\
%             Add $\Gamma'$ as a child of $\Gamma$.
%         }
%     }
%     \ElseIf{ there is a leaf in $\mathcal{T}$ that has no $\bot$ term, is  saturated against Propositional and Survival Rules but not saturated against Knowledge Rules}{
%         Let the leaf be $\Gamma$ and $(\sigma\ \ w\ \ \psi)$ be a Knowledge unsaturated term.\\
%         $\Gamma' = \Gamma$\\
%         \If{$\psi = K\chi$}{
%             $\Gamma' = \Gamma'\union\{(\sigma'\ \ w\ \ \chi)\mid \{(\sigma,\sigma'), (\sigma'\ \ w\ \ \checkmark)\}\subseteq\Gamma\}$\\
%             Add $\Gamma'$ as a child of $\Gamma$.
%         }
%         \ElseIf{$\psi = \hat{K}\chi$}{
%             $\Gamma' = \Gamma'\union\{(\sigma_n, \sigma_n), (\sigma_n\ \ w\ \ \checkmark), (\sigma_n\ \ w\ \ \chi)\}\union\{(\sigma', \sigma_n), (\sigma_n, \sigma')\mid (\sigma'\ \ w\ \ \checkmark)\in\Gamma\}$\\
%             Add $\Gamma'$ as a child of $\Gamma$.
%         }
%     }
%     \ElseIf{there is a leaf in $\mathcal{T}$ that has no $\bot$ term, is  saturated against Propositional, Survival Rules and Knowledge Rules, but not saturated against Diamond and Box Rules}{
%         Let $\Gamma$ be the unsaturated leaf and $(\sigma\ \ w\ \ \psi)$ be the unsaturated term\\
%         $\Gamma' = \Gamma$
%         \If{$\psi = [w']\chi$ where $|w'| > 1$ and $w' = aw''$ where $a\in\Sigma$}{
%             $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ [a][w'']\chi)\}$\\
%             Add $\Gamma'$ as a child of $\Gamma$
%         }
%         \ElseIf{$\psi = \ldiaarg{w'}\chi$ where $|w'| > 1$ and $w' = aw''$ where $a\in\Sigma$}{
%             $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ \ldiaarg{a}\ldiaarg{w''}\chi)\}$
%         }
%     }
% }
% Return UNSAT
% % \end{algorithmic}
% \end{algorithm}

% \newpage
Given a formula $\varphi$:
\begin{enumerate}
    \item Let $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$

    \item Let$\mathcal{T}$ be a tree of set of terms of tableau with $\Gamma$ in the root.
    
    \item While there is a case matching from $(a)$ to $(c)$ and new terms can be inferred:
    \begin{enumerate}
        \item there is a leaf in $\mathcal{T}$ that has no $\bot$ term and it is not saturated against Propositional and Survival Rules then :
        \begin{enumerate}
            \item Let $\Gamma$ be the leaf.
            \item Let $(\sigma\ \ w\ \ \psi)$ or $(\sigma\ \ w\ \ \checkmark)$ be the term that are unsaturated.
            \item $\Gamma' = \Gamma$
            \item If $\psi = l$ where $l$ is of the form either $p$ or $\neg p$, where $p$ is a propositional letter then
            \begin{enumerate}
                \item $\Gamma' = \Gamma'\union \{(\sigma\ \ w\ \ [a]\psi), (\sigma\ \ \epsilon\ \ \psi)\}$, by Constant valuation if and Up
                \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
            \end{enumerate}
            
            \item Else If $\psi = \psi_1\wedge\psi_2$ then 
            \begin{enumerate}
                \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ \psi_1), (\sigma\ \ w\ \ \psi_2)\}$
                \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
            \end{enumerate}
        
            \item Else If $\psi = \psi_1\vee\psi_2$ then 
            \begin{enumerate}
                \item $\Gamma'_1 = \Gamma'\union\{(\sigma\ \ w\ \ \psi_1)\}$
                
                \item $\Gamma'_2 = \Gamma'\union\{(\sigma\ \ w\ \ \psi_2)\}$
                
                \item Add $\Gamma'_1$ and $\Gamma'_2$ as children of $\Gamma$ in $\mathcal{T}$.
            \end{enumerate}
            
        
            \item Else If $\{(\sigma\ \ w\ \ \psi), (\sigma\ \ w\ \ \neg\psi)\}\subseteq\Gamma$ then
            \begin{enumerate}
                \item  $\Gamma' = \Gamma'\union\{\bot\}$
                \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
            \end{enumerate}
           
            \item Else
            \begin{enumerate}
                \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w'\ \ \checkmark)\mid w'\in Pre(\LL(w))\}$
                
                \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
            \end{enumerate}
        \end{enumerate}
        
        \item Else If there is a leaf in $\mathcal{T}$ that has no $\bot$ term, is  saturated against Propositional and Survival Rules but not saturated against Knowledge Rules then 
        \begin{enumerate}
            \item Let the leaf be $\Gamma$ and $(\sigma\ \ w\ \ \psi)$ be a Knowledge unsaturated term.
            
            \item $\Gamma' = \Gamma$
            
            \item If $\psi = K\chi$ then
            \begin{enumerate}
                \item $\Gamma' = \Gamma'\union\{(\sigma'\ \ w\ \ \chi)\mid \{(\sigma,\sigma'), (\sigma'\ \ w\ \ \checkmark)\}\subseteq\Gamma\}$
                
                \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
            \end{enumerate}
            
            \item Else If $\psi = \hat{K}\chi$ then 
            \begin{enumerate}
                \item $\Gamma' = \Gamma'\union\{(\sigma_n, \sigma_n), (\sigma_n\ \ w\ \ \checkmark), (\sigma_n\ \ w\ \ \chi)\}\union\{(\sigma', \sigma_n), (\sigma_n, \sigma')\mid (\sigma'\ \ w\ \ \checkmark)\in\Gamma\}$
                
                \item  Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
            \end{enumerate}
        \end{enumerate}
        \item Else if there is a leaf in $\mathcal{T}$ that has no $\bot$ term, is  saturated against Propositional, Survival Rules and Knowledge Rules, but not saturated against Diamond and Box Rules then
        \begin{enumerate}
            \item Let $\Gamma$ be the unsaturated leaf and $(\sigma\ \ w\ \ \psi)$ be the unsaturated term
            
            \item $\Gamma' = \Gamma$
            \item If $\psi = [w']\chi$ where $|w'| > 1$ and $w' = aw''$ where $a\in\Sigma$ then 
            \begin{enumerate}
                \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ [a][w'']\chi)\}$
                
                \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
            \end{enumerate}
            \item Else If $\psi = \ldiaarg{w'}\chi$ where $|w'| > 1$ and $w' = aw''$ where $a\in\Sigma$ then
            \begin{enumerate}
                \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ \ldiaarg{a}\ldiaarg{w''}\chi)\}$
                
                \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
            \end{enumerate}
            
            \item Else If $\psi = \ldiaarg{a}\chi$ then
            \begin{enumerate}
                \item $\Gamma' = \Gamma'\union\{(\sigma\ \ wa\ \ \chi), (\sigma\ \ wa\ \ \checkmark), (\sigma\ \ w\ \ [a]\chi)\}$
                
                \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
            \end{enumerate}
            
            \item Else If $\psi = [a]\chi$ and $(\sigma\ \ wa\ \ \checkmark)\in\Gamma$ then
            \begin{enumerate}
                \item $\Gamma' = \Gamma\union\{(\sigma\ \ wa\ \ \chi)\}$
                
                \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
            \end{enumerate}
        \end{enumerate}
    \end{enumerate}
    
    \item Traverse through the leaves of $\mathcal{T}$.
    \item If there is a leaf with no $\bot$ in it, return SAT, else UNSAT.
\end{enumerate}

For the rest of the paper, we refer that $\mathcal{T}$ that is created as the tableau tree. Similarly as above, if there is a path from root of $\mathcal{T}$ to a leaf that has no $\bot$ in it, this tree is said to be open (intuitively indicating tableau to be open), else it is closed.
\subsubsection{Termination}
Before proving termination, let us define an important notion of Fischer Ladner Closure of a formula.
\begin{defi}
\textbf{Fischer-Ladner Closure} The Fisher-Ladner closure of a formula $\varphi$ , denoted $FL(\varphi)$, is the minimal set satisfying
    \begin{itemize}
        \item $\varphi\in FL(\varphi)$
        \item if $\psi\in FL(\varphi)$ then $\neg\psi \in FL(\varphi)$, provided $\psi$ does not start with $\neg$
        \item if $\neg\psi, \psi\wedge\chi, K\psi$ or $[\pi]\psi$ are in $FL(\varphi)$ then $\psi,\chi \in FL(\varphi)$
        \item if $[\pi_1;\pi_2]\psi \in FL(\varphi)$ then $[\pi_1][\pi_2]\psi \in FL(\varphi)$
        \item if $[\pi_1+\pi_2]\psi \in FL(\varphi)$ then both $[\pi_1]\psi$ and $[\pi_2]\psi$ are in $FL(\varphi)$
        \item if $[\pi^{\star}]\psi \in FL(\varphi)$ then $[\pi][\pi^\star]\psi \in FL(\varphi)$
    \end{itemize}
\end{defi}
\begin{theorem}
Given the formula $\varphi$, the tableau proof for satisfiability terminates.
\label{lemma:terminationwordone}
\end{theorem}
\begin{proof}
We can prove that a term like $(\sigma\ \ w\ \ \varphi)$, for any $w$ and any $\sigma$, the tableau proof for $\{(\sigma\ \ w\ \ \varphi), (\sigma,\sigma), (\sigma\ \ w\ \ \checkmark)\}$ terminates, by induction on the size of $\varphi$.

\textbf{Base Case.} Consider the case where $\varphi = p$ where $p$ is a propositional letter. Starting from $\Gamma = \{(\sigma\ \ w\ \ \varphi), (\sigma,\sigma), (\sigma\ \ \epsilon\ \ \checkmark)\}$, the tableau applies constant valuation rule $|\Sigma|$ times and then the tableau terminates here since no more rule can be applied.

\textbf{Induction Hypothesis.} Let the statement be true any $\varphi$ such that $|\varphi| = n$.

\textbf{Induction Step.} Consider $\varphi$ such that $|\varphi| = n + 1$. We go case by case in syntax of $\varphi$:
\begin{itemize}
    \item $\varphi = \psi\wedge\chi$. Here, the AND rule gets applied to produce $(\sigma\ \ w\ \ \psi)$ and $(\sigma\ \ w\ \ \chi)$, and by IH proof for them terminates.
    
    \item $\varphi = \psi\vee\chi$. Here the OR rule will give $(\sigma\ \ w\ \ \psi)$ or $(\sigma\ \ w\ \ \chi)$ which again is terminating.
    
    \item $\varphi = K\psi$. By the knowledge rule , the term $(\sigma \ \ w\ \ \psi)$ (We start by $(\sigma,\sigma)$). By IH, this terminates.
    
    \item $\varphi = \hat{K}\psi$. By the possibility rule, we introduce a new label $\sigma_n$ and term $(\sigma_n\ \ w\ \ \psi)$ as well as the relational terms and the survival terms $(\sigma_n\ \ w\ \ \checkmark)$. The Survival Chain rule hence adds $|w|$ many checkmark terms. Also, since by IH, number of unique previously produced world labels are finite, say $l$, hence the relational terms for $\sigma_n$ adds $l$ more relation terms. By IH, proof for this terminates.
    
    \item $\varphi = \ldiaarg{a\pi}\psi$. By the diamond decompose we derive $(\sigma\ \ w\ \ \ldiaarg{a}\ldiaarg{\pi}\psi)$ and by diamond project, we derive $(\sigma\ \ wa\ \ \checkmark)$ and $(\sigma\ \ wa\ \ \psi)$. By IH, the proof for this terms terminate.
    
    \item $\varphi = [a\pi]\psi$. By box decompose, we derive $(\sigma\ \ w\ \ [a][\pi]\psi)$. If term $(\sigma\ \ wa\ \ \checkmark)$ already derived, by box project $(\sigma\ \ wa\ \ [\pi]\psi)$ is derived, and by IH, the proof for this term terminates.
\end{itemize}

Now for every $\hat{K}$, there arrives a new label $\sigma'$, and for every $\ldiaarg{a}$ operator, a letter gets added in $w$. Hence $\#\sigma$ is finnite since $\varphi$ is finite, where $\#\sigma$ is number of unique world labels. Also since max legnth of such a $w$ is at most $O(|\varphi|)$, because of survival chain, there can be $|w|$ many terms derived and hence polynomial to size of $|\varphi|$ such terms. Since there can be at most $\Sigma^{O(|\varphi|)}$ such unique words, hence the proof terminates, that is arrives at a point where it cannot derive more new terms.
\end{proof}
% \begin{theorem}
% The Satisfiability problem of single agent word fragment of $\POL$ is $\NP$-Complete. (?)
% \end{theorem}
% \begin{proof}
% We prove the satisfiability to be in $\NP$ using the tableau proof system algorithm presented above. Since Propositional Logic is a special case of $\POL_1$, satisfiability of $\POL_1$ is hence $\NP$-Hard.

% % Given $\varphi$, let $\mathcal{T}$ be the tableau tree from the root $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma, \sigma)\}$.

% % Now we prove the following statement:

% % \textbf{Given a node $\Gamma$ in $\mathcal{T}$ such that $|\Gamma| = n$, the size of its child $|\Gamma_1|\leq O(n^c)$ for some constant $c$.}

% % \begin{proof}
% % We start with the root node. Here $|\Gamma| = 3$. There are 14 rules. 

% % Since this is the root node, if $\varphi = \ldiaarg{w}\psi$, hence by Decomposition rule, it adds $\ldiaarg{a}\ldiaarg{w'}\psi$ ($w = aw'$), and further applies Diamond Project, which adds 1 term, and by Survival chain, it adds at most 1 term since only single letter has been considered. Hence in the child, there can be at most $14\times 4\times 3$ terms added (a rule can at max add 4 terms, there are 14 rules and $\Gamma$ has 3 terms), which polynomial to $3$ (number of rules and number of terms a rule can add here is constant).


% % Let $|\Gamma| = n$. Consider every rule except survival chain. Similarly like previous root case, each term can add at most $13\times 4 = 42$ terms. Hence $n$ terms can contribute at most $42n$ terms in child. 

% % Now we move on to Survival Chain. Let us assume there is a term $(\sigma\ \ w\ \ \hat{K}\psi)$, hence this creates a $(\sigma'\ \ w\ \ \psi)$ and also include term $(\sigma'\ \ w\ \ \checkmark)$. By survival chain rule, this adds $|w|$ new terms. $|w|\leq |\varphi|$. Hence this adds, in total, at most $42n^2$ terms.
% % \end{proof}

% % \textbf{PROBLEM}: Now even if we prove the depth of the tree $\mathcal{T}$ to be linear in $|\varphi|$, the size in the leaf node hence blows up to be exponential.
% Now consider the leaf node $\Gamma_l$ of $\mathcal{T}$. Wlog, assume $\bot\notin \Gamma_l$.

% Each term is of the form $(\sigma\ \ w\ \ \varphi), (\sigma\ \ w\ \ \checkmark)$ or $(\sigma, \sigma')$. For every possibility rule we introduce a $(\sigma, \sigma')$ and a new label $\sigma$. Hence number of unique $\sigma$ appearing in the leaf node $\Gamma_l$, as well as $(\sigma,\sigma')$ for every $\sigma$, is linear to the number of $\hat{K}$ operators in $\varphi$. Hence total number of possible $(\sigma,\sigma')$ terms are quadratic to the number of $\hat{K}$ operators in $\varphi$.

% For every instance rule except the survival chain rules, the project determinism and clash rule, the formula $\chi$ in the denominator is in the $FL(\psi)$, where $\psi$ is the formula in one of the terms in numerator. Hence number of possible formula is $|FL(\varphi)|\leq |\varphi|$.

% Now only thing left to prove is number of $w$'s possible. We start with $\epsilon$. From the instance rule, given a term $(\sigma\ \ w\ \ \varphi)$, only way a letter $a\in\Sigma$ is added in $w$ and contributes a term of the form $(\sigma\ \ wa\ \ \psi)$, is because of a term $(\sigma\ \ w\ \ \ldiaarg{a}\psi)$. Hence number of largest $w$'s such that there is no $w'\in\LL(Pre(w))$ is again at most polynomial to the size of $\varphi$.

% Hence we prove $\Gamma_l$ is of size polynomial with respect to $|\varphi|$. To verify whether this set is a certificate for the satisfiability of $\varphi$, we just have verify whether this set is saturated. By completeness, we know that a satisfying model can be created.

% To check saturation, we take each tableau term $t\in\Gamma_l$, we verify whether all the terms that can be derived from $t$ is in $\Gamma_l$ along with the assumptions (such that for box formula, we have to check whether a survival term is already there). There are constant inference rules in tableau, let it be $c$. $|\Gamma_l| = P(|\varphi|)$, where $P(X)$ is a polynomial of $X$. Hence steps to verify saturation is : at most $P(X)\times 4c$ to check membership of the consequence for each term (the 4 since a rule can at most derive 4 terms). Therefore total steps is at most $[P(|\varphi|)]^2\times 4c$.
% \end{proof}


\subsubsection{Soundness and Completeness}
\begin{theorem}
Given a formula $\varphi$, if $\varphi$ is satisfiable, then the tableau for $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$ is open.
\end{theorem}
\begin{proof}
We prove that if $\varphi$ is satisfiable then there exists a subtree rooted at some child $\Gamma_c$ of the root $\Gamma$ in $\mathcal{T}$ which is open using induction on the depth of the tableau tree $\mathcal{T}$. Let the pointed epistemic model that satisfy $\varphi$ be $\M,s$.

\textbf{Base Case.} Let the base case be $|\Gamma| = 3$. Since we start from $\{(\sigma\ \ \epsilon\ \ \varphi), (\sigma, \sigma), (\sigma\ \ \epsilon\ \ \checkmark)\}$. Hence this implies $\varphi = l$ or $\varphi = [a]\psi$, where $l$ is a literal (a positive propositional letter or a negation of it). Hence the tableau remains open since no $\bot\in\Gamma$.

\textbf{Induction Hypothesis.} Let the statement be true for any tableau tree $\mathcal{T}$ of depth at most $n$.

\textbf{Inductive Step.} Consider the tableau tree $\mathcal{T}$ rooted at $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma, \sigma), (\sigma\ \ \epsilon\ \ \checkmark)\}$ of depth at most $n + 1$. Now we go case by case with $\varphi$:
\begin{itemize}
    \item $\varphi = \psi\wedge\chi$: We apply AND rule, and hence $\Gamma' = \Gamma\union\{(\sigma\ \ \epsilon\ \ \psi), (\sigma\ \ \epsilon\ \ \chi)\}$, which is a child rooted at $\Gamma$. Since $\M,s\vDash\varphi$, by definition $\M,s\vDash\psi$ and $\M,s\vDash\chi$. By IH, tableau tree rooted at $\Gamma'$ is open, which suggestes, $\mathcal{T}$ is open.
    
    \item $\varphi = \psi\vee\chi$: We apply OR rule and hence we get two children, $\Gamma_1 = \Gamma\union\{(\sigma\ \ \epsilon\ \ \psi)\}$ and $\Gamma_2 = \Gamma\union\{(\sigma\ \ \epsilon\ \ \chi)\}$. Since $\M,s\vDash\psi\vee\chi$, hence $\M,s\vDash\psi$ or $\M,s\vDash\chi$. By IH, one of the sub tableau tree rooted at $\Gamma_1$ or $\Gamma_2$ will be open, hence implying $\mathcal{T}$ to be open.
    
    \item $\varphi = K\psi$: By applying the Knowledge rule, $\Gamma' = \Gamma\union\{(\sigma'\ \ \epsilon\ \ \psi)\mid \{(\sigma, \sigma'), (\sigma'\ \ \epsilon\ \ \checkmark)\}\subseteq\Gamma\}$. Since $\M,s\vDash K\psi$, hence for every $s'\in\M$ such that $s\sim s'$, $\M,s'\vDash\psi$. By IH, the tableau subtree rooted at $\Gamma'$ is open.
    
    \item $\varphi = \hat{K}\chi$: By applying the possibility rule, $\Gamma' = \Gamma\union\{(\sigma_n, \sigma_n), (\sigma_n\ \ \epsilon\ \ \checkmark), (\sigma_n\ \ \epsilon\ \ \chi)\}\union\{(\sigma', \sigma_n), (\sigma_n, \sigma')\mid (\sigma'\ \ \epsilon\ \ \checkmark)\in\Gamma\}$. Since, $\M,s\vDash\hat{K}\chi$, hence there is an $s_n\in\M$ such that $\M,s_n\vDash\chi$, also $s_n\sim s'$ for every $s'\in\M$ since $\sim$ is an equivalence relation. Hence by IH, the sub tableau tree rooted at $\Gamma'$ is open.
    
    \item $\varphi = \ldiaarg{w}\psi$: Consider $w = aw'$. Hence by the diamond decomposition rule $\Gamma' = \Gamma\union\{(\sigma\ \ \epsilon\ \ \ldiaarg{a}\ldiaarg{w'}\psi)\}$. Since $\M,s\vDash\ldiaarg{aw'}\psi$, hence $\M|_{aw'},s\vDash\psi$, which also suggests, $\M|_a,s\vDash\ldiaarg{w'}\psi$, which implies $\M,s\vDash\ldiaarg{a}\ldiaarg{w'}\psi$. Now consider $w = a$. Hence now by Projection rule, $\Gamma' = \Gamma\union\{(\sigma\ \ a\ \ \checkmark), (\sigma\ \ a\ \ \psi)\}$. Since $\M,s\vDash\ldiaarg{a}\psi$, therefore $s\in\M|_a$ and $\M|_a,s\vDash\psi$.
    
    Hence in both the cases for $w = aw'$ or $w = a$, by IH, the sub tableau tree rooted at $\Gamma'$ is open. The proof goes similarly for box.
\end{itemize}
\end{proof}

\begin{theorem}
Given a formula $\varphi$, if the tableau for $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$ is open, then $\varphi$ is satisfiable.\label{theorem:wordonecomplete}
\end{theorem}
\begin{proof}
Since by assumption, the tableau for $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$ is open, there exists a branch in the tableau tree where in the leaf node there is  a set of terms $\Gamma_l$ such that it is saturated and $\bot\notin\Gamma_l$.

For the purpose of this proof, let us define a relation over the words $\bar{w}$ that appears in $\Gamma_l$. For any two word $\bar{w}_1$ and $\bar{w}_2$ that appears in $\Gamma_l$, $\bar{w}_1\leq_{pre}\bar{w}_2$ if and only if $\bar{w}_1\in\LL(Pre(\bar{w}_2))$. Now, this relation is reflexive ($\bar{w}_1\in\LL(Pre(\bar{w}_1))$), asymmetric (if $\bar{w}_1\in\LL(Pre(\bar{w}_2))$ and $\bar{w}_2\in\LL(Pre(\bar{w}_1))$ then $\bar{w}_1 = \bar{w}_2$) and transitive (if $\bar{w}_1\in\LL(Pre(\bar{w}_2))$ and $\bar{w}_2\in\LL(Pre(\bar{w}_3))$ then $\bar{w}_1\in\LL(Pre(\bar{w}_3))$). Hence this relation creates a partial order among all the words occuring in $\Gamma_l$. We also denote $\bar{w_1}<_{pre}\bar{w_2}$ to interpret the fact that $\bar{w_1}\leq_{pre}\bar{w_2}$ and $\bar{w_1}\neq\bar{w_2}$.

Now we create a model $\M = \ldiaarg{W, R, V, Exp}$ out of $\Gamma_l$ and prove that $\varphi$ is satisfied by some world in the model.

\begin{itemize}
    \item $W = \{s_\sigma\mid \sigma\mbox{ is a distinct label in the terms occuring in }\Gamma_l\}$
    
    \item $R = \{\{s_{\sigma_1}, s_{\sigma_2}\}\mid(\sigma_1,\sigma_2)\in\Gamma_l\}$
    
    \item $V(s_\sigma) = \{p\mid (\sigma\ \ \epsilon\ \ p)\in\Gamma_l\}$
    
    \item $Exp(s_\sigma) = \sum_{w\in\Lambda_\sigma}w$, where $\Lambda_\sigma = \{w\mid (\sigma\ \ w\ \ \checkmark)\in\Gamma_l\mbox{ and }\nexists w':((\sigma\ \ w'\ \ \checkmark)\in\Gamma_l\mbox{ and }w<_{pre} w')\}$
\end{itemize}

Note that, new world label $\sigma_n$ is only created in the possibility rule, with a reflexive relation on itself. Now consider the set $R' = \{(\sigma, \sigma')\mid \{(\sigma\ \ \epsilon\ \ \checkmark), (\sigma' \ \ \epsilon\ \ \checkmark)\}\subseteq\Gamma_l\}$. Hence this can be considered a binary relation over the set of all distinct $\sigma$ that occurs in $\Gamma_l$. When a $\sigma'$ is created by possibility rule, it is reflexive. Also by the relation rules in possibility rule, they are made symmetrically related with every other label that has been previously there. Also, if a $\sigma'$ is created with term $(\sigma'\ \ w\ \ \checkmark)$, by Survival Chain the term $(\sigma'\ \ \epsilon\ \ \checkmark)$ also gets included. Hence $R'$ is an equivalence relation, hence making $R$ in the model an equivalence relation.


Now we shall prove the following two statement:

\textbf{If $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$ then $s_{\sigma}$ survives in $\M|_w$}

and 

\textbf{If $(\sigma\ \ w\ \ \varphi)\in\Gamma_l$ and $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$ then $s_{\sigma}$ survives in $\M|_w$ and  $\M|_w,s_\sigma\vDash\varphi$}.


For the first statement, we induct on the size of $|w|$.

\textbf{Base Case.} Let $|w| = 1$. Hence $w \in \{\epsilon\}\union \Sigma$ . Since $\Gamma\subseteq\Gamma_l$ and $(\sigma\ \ \epsilon\ \ \checkmark)$, and $s_\sigma$ is in $\M|_\epsilon = \M$.

For the case $w = a$ for any $a\in\Sigma$. Hence there exists a word $w'$ that occurs in a term in $\Gamma_l$ labelled by $\sigma$ such that $w\in\LL(Pre(w'))$ and there is no other word bigger than $w'$ such that $w'$ is in its prefix, since by lemma \ref{lemma:terminationwordone}, the proof terminates. Hence by definition of $w'\in\LL(Exp(s_\sigma))$ which guarantees survival of $s_\sigma$ in $\M|_a$. 

\textbf{Induction Hypothesis.} Assume the statement to be true for $|w| = n$.

\textbf{Inductive Step.} Consider the case where $|w| = n + 1$. 

By assumption, $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$. Hence by the fact that $\Gamma_l$ is saturation and by rule "Survival Chain", there is $(\sigma\ \ w'\ \ \checkmark)\in\Gamma_l$, where $w = w'a$ for some $a\in\Sigma$. Hence by IH, the result follows that $s_\sigma$ survives in $\M|_{w'}$. 

Now, by termination, there are finite many unique words occuring in $\Gamma_l$. Clearly, $w'\leq_{pre} w$. Since there are finite many words, there is a $w_*$, which is of maximum size such that $w\leq_{pre} w_*$ and $(\sigma\ \ w_*\ \ \checkmark)\in\Gamma_l$. Hence $w_*\in\Lambda_\sigma$ in the definition of Exp of model. Therefore $w_*\in\LL(Exp(s_\sigma))$ and since $w'\leq_{pre} w\leq_{pre} w_*$, $s_\sigma$ survives in $\M|_{w'}$, hence $s_\sigma$ shall survive in $\M|_{w}$.

% Now, since $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$, there is a $w''$ occurring in a term of form $(\sigma\ \ w''\ \ \checkmark)\in\Gamma_l$  such that $w\in \LL(Pre(w''))$ and there is no $w'''$ such that $(\sigma\ \ w'''\ \ \checkmark)\in\Gamma_l$ and $w''\in\LL(Pre(w'''))$. Hence, by definition of the model ($Exp$), $w''\in\Lambda$, which further suggests $w''\in\LL(Exp(s_\sigma))$. Since $w\in\LL(Pre(w''))$ and $s_\sigma$ is in $\M|_{w'}$, therefore $s_\sigma$ survives in $\M|_{w}$. This proves the first part of the proof that if $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$, then $s_\sigma$ survives in $\M|_w$.

\textbf{Proof for Second Statement.}
Naturally, we shall induct upon the size of $w$ and $\varphi$. But the induction is such that the we assume hypothesis for larger $w$ and smaller $\varphi$, and we prove statement for smaller $w$ and larger $\varphi$. That is, let the statement be $\mathcal{P}(m, n)$, where $m = |w|$ and $n = |\varphi|$, assuming this we try proving $\mathcal{P}(m',n')$, where $m'\leq m$ and $n\geq n'$.

\textbf{Base Case.} Let $|w| = m$, where $m$ is maximum among all the size of words occurring in the terms of $\Gamma_l$. Therefore, $\varphi$ is not of the form $\ldiaarg{w}\psi$, where $w$ is a word over $\Sigma$, as $\Gamma_l$ is saturated. We prove it step by step on syntax of $\varphi$.
\begin{itemize}
    \item (Base Case for $\varphi$ in $m$), $\varphi = p$. Since $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$ hence $s_\sigma$ survives in $\M|_w$. Also, by constant valuation up, $(\sigma\ \ \epsilon\ \ p)\in\Gamma_l$. Hence By definition of model, $\M|_w,s_{\sigma}\vDash p$. Similar for negation.
    
    \item $\varphi = \hat{K}\psi$. Since $\Gamma_l$ is saturated, by the rule of possibility, $\{(\sigma'\ \ w\ \ \psi), (\sigma, \sigma'), (\sigma'\ \ w\ \ \checkmark)\}\subseteq\Gamma_l$. By IH on the subformula of $\varphi$, definition of model, the proof of previous statement, and the rule "survival chain", $s_{\sigma'}$ survives in $\M|_{w}$ and $\M|_w,s_{\sigma'}\vDash\psi$. Also by definition, $\{s_{\sigma}, s_{\sigma'}\}\in R$, hence proving $\M|_w, s_\sigma\vDash\hat{K}\psi$.
    
    \item $\varphi = K\psi$. Since $\Gamma_l$ is saturated, and by previous statement $s_{\sigma'}$ is surviving for every $(\sigma'\ \ w\ \ \checkmark)$, by the rule of knowledge $(\sigma'\ \ w\ \ \psi)\in\Gamma_l$ for every $(\sigma, \sigma')$. Hence by IH on subformula, $\M|_w, s_{\sigma'}\vDash\psi.$
    
    \item $\varphi = [w']\psi$. Since $m$ is the biggest, there is no $(\sigma\ \ wa\ \ \checkmark)\in\Gamma_l$ and hence vacuously, $\M|_w,s_\sigma\vDash[a]\psi$.
    
\end{itemize}

\textbf{Induction Hypothesis.} Let us consider the statement is true for any $w$ and $\varphi$ such that $|w|>m'$ and $|\varphi|<n'$ for some $m'$ and $n'$.

\textbf{Inductive Step.} We prove for $|w| = m'$ and $|\varphi| = n'$. Again, we go case by case on syntax of $\varphi$. The cases proof for every syntax other than $\ldiaarg{a}\psi$ is same as previous.

Hence let $\varphi = \ldiaarg{a}\psi$. Since $\Gamma_l$ is saturated, $\{(\sigma\ \ wa\ \ \checkmark), (\sigma\ \ wa\ \ \psi)\}\subseteq\Gamma_l$ by the diamond rule. By the proof of the previous statement, $s_\sigma$ survives in $\M|_{wa}$. Also by IH on $|w|$ as well as $|\varphi|$, $\M|_{wa},s_\sigma\vDash\psi$. Hence, $\M|_w,s_\sigma\vDash\ldiaarg{a}\psi$.

Similar proof goes for box.
\end{proof}

\subsection{Proof For NP-Completeness for Word Single Agent}
\begin{theorem}
A formula $\varphi$ is word $\POL_1$ satisfiable iff it can satisfied by a model of at most $O(|\varphi|)$ worlds, each having expectation of size at most $O(p(|\varphi|))$, where $p(X)$ is some polynomial in $X$.
\label{theorem:wordonesmall}
\end{theorem}
\begin{proof}
Assuming there is a model of at most $O(|\varphi|)$ worlds, proving $\varphi$ is satisfiable is trivial.

We prove the converse. We assume that $\varphi$ is satisfiable. Since it is satisfiable, we can build a model $\M$ from its open tableau just like we created in proof of theorem \ref{theorem:wordonecomplete}. Consider the $\M = \ldiaarg{W, R, V, Exp}$ and say $\M,s\vDash\varphi$. Note that, $\varphi$ is in negation normal form. First we partition the set $W$ using the following equivalence relation $\equiv$:
\begin{itemize}
    \item $s\equiv s$.
    \item $s'\equiv s''$, for every $s',s''\neq s$, iff for $\hat{K}\psi\in FL(\varphi)$, $\M,s'\vDash\psi$ and $\M,s''\vDash\psi$
\end{itemize}

Let us denote the partition by $\equiv$ as $s_\varphi = [s]_\equiv$, where $\M,s\vDash\varphi$ and $s_\psi = [s']_\equiv$ where for any $s'\in [s']_\equiv$, there is some $\hat{K}\psi\in FL(\varphi)$ such that $\M,s'\vDash\psi$.

Now we create a model $\M' = \{W', R', V', Exp'\}$ as following:
\begin{itemize}
    \item $W' = \{s_\varphi\}\union \{s_\psi\mid \hat{K}\psi\in FL(\varphi)\}$.
    \item $R' = \{(s_\psi,s_{\psi'})\mid s_\psi\in W', s_{\psi'}\in W'\}$
    \item $V'(s_\psi) = V(s')$ where $s'\in s_\psi$.
    \item $Exp'(s_\varphi) = Exp(s)$.
    
    $Exp'(s_\psi) = \sum_{s'\in s_\psi} Exp(s')$.
\end{itemize}


Now we shall prove for any $w\in\Sigma^*$ occuring in tableau of $\varphi$, for any $\psi\in FL(\varphi)$, for any $s'\in W'$
\begin{align*}
    \exists s''\in s' &\M|_w,s''\vDash\psi\\
                    &\mbox{ iff }\\
                    \M'|_w,&s'\vDash\psi
\end{align*}
We induct on the size of $\psi$.

\textbf{Base Case.} The case of $\psi = p$ or $\psi = \neg p$, where $p$ is a propositional letter. By definition of $V'$ in the definition of $\M'$, the result holds.

\textbf{Induction Hypothesis.} Let the statement be true for any $\psi$ of size at most $n$.

\textbf{Inductive Step.} Consider $\psi$ such that $|\psi| = n + 1$.
\begin{itemize}
    \item $\psi = \hat{K}\chi$. Assume there is a $s_1\in s'$ such that $\M|_w,s_1\vDash\hat{K}\chi$, which implies there is a $t\in W$ such that $\M|_w,t\vDash\chi$. 
    
    Now $\hat{K}\chi\in FL(\varphi)$, and since the $\M$ is complete (every world is related to every other world), $\M|_w,s\vDash\hat{K}\chi$, where $s\in s_\varphi$ (since $\varphi$ is assumed satisfiable, hence $s$ is surviving in $\M|_w$). Therefore, by the partition definition (definition of the equivalence relation), there is a partition $s_\chi$ such that $t\in s_\chi$.
    
    By IH, $\M'|_w, s_\chi\vDash$ and hence $\M'|_w,s'\vDash\hat{K}\chi$.
    
    Conversely, let $\M'|_w, s'\vDash\hat{K}\chi$. Hence there is a $t'\in W'$ where $\M'|_w,t'\vDash\chi$. By IH, there is a $t\in t'$ such that $\M|_w,t\vDash\chi$. Since $\M$ is a complete model, $\M|_w,s\vDash\hat{K}\psi$.
    
    Similarly can be proven for $\psi = K\chi$.
    
    \item $\psi = \ldiaarg{a}\chi$. Note that we ignore $\psi = \ldiaarg{aw}\chi$, where $w\in\Sigma^*$ since $\M|_w,s'\vDash\ldiaarg{aw}\chi$ if and only if $\M|_w,s'\vDash\ldiaarg{a}\ldiaarg{w}\chi$.
    
    Let us assume $\M|_w, s_1\vDash\ldiaarg{a}\chi$ for some $s_1\in s'$. Now two cases are possible, $s' = s_\varphi$, which implies $s_1 = s$. By assumption, $\M|_{wa}, s_1\vDash\chi$. By definition, $Exp'(s_\varphi) = Exp(s_1)$. Hence, since $s_1$ is surviving after projection on $wa$, $s_\varphi$ shall also survive after projection on $wa$. By IH, $\M'|_{wa}, s_\varphi\vDash\chi$, which implies $\M'|_w,s_\varphi\vDash\ldiaarg{a}\chi$.
    
    Another case that is possible is $s'\neq s_\varphi$. In that case, by the definition of $Exp'(s')$, $\LL(Exp(s_1))\subseteq \LL(Exp(s'))$. Hence in this case too, $s'$ survives the projection on $wa$. And hence, similarly by IH, our statement holds true.
    
    Conversely, let $\M'|_w, s'\vDash\ldiaarg{a}\chi$. Note that, by definition of the Expectation function, $\LL(Exp'(s')) = \bigcup_{s_0\in s'}\LL(Exp(s_0))$. By assumption $\M'|_{wa},s'\vDash\chi$. By the definition of Expectation function, there exists some $w'\in\bigcup_{s_0\in s'}\LL(Exp(s_0))$ for which $s'$ survives the projection on $wa$, that is $wa\in\LL(Pre(w'))$. Therefore there is some world $s_1\in s'$, which survives the projection and by IH, $\M|_{wa}, s_1\vDash\chi$, which gives us the required result.
    
    Similarly can be proven for Box modality.
\end{itemize}

Also in the model $\M'$ we created, each world $s_\psi$ has Expectation such that $w\in\LL(Exp'(s_\psi))$ means $w$ has occurred in some term of the form $(\sigma\ \ w\ \ \checkmark)$ in the tableau proof for satisfiability. The size of such $w$ is at most $|\varphi|$ since $w$ gains one letter that $\varphi$ loses from its diamond operator. Also number of such maximal $w$'s (there is no $w'$ which has $w$ as prefix) will also be at most $|\varphi|$. Hence $|Exp'(s_\psi)|\leq O(q(|\varphi|))$ for some polynomial $q$.
\end{proof}

\begin{corollary}
The satisfiability problem of single agent word fragment of $\POL$ is $\NP$-Complete.
\end{corollary}
\begin{proof}
By theorem \ref{theorem:wordonesmall}, for any formula $\varphi$ of single agent word fragment of $\POL$, $\varphi$ is word $\POL_1$ satisfiable iff it can satisfied by a model of at most $O(|\varphi|)$ worlds, each having expectation of size at most $O(p(|\varphi|))$, where $p(X)$ is some polynomial in $X$.

Since model checking of word fragment is in $P$, satisfiability of word fragment of $\POL_1$ is in $\NP$.

Also, propositional satisfiability is a special case of this decision problem, hence that makes this problem $\NP$-Complete.
\end{proof}

==> tableau1-starfee.tex <==
Here, in this section, we design a proof system using tableau method to prove satisfiability. Each tableau term is of the form $(\sigma\ \ w\ \ \varphi)$ or $(\sigma\ \ w\ \ \checkmark)$ or $(\sigma_1,\sigma_2)$, where $w\in\Sigma^*$, $\varphi\in\POL_1$ and $\sigma, \sigma_1, \sigma_2$ are labels. 

Intuitively, each label represents a world in the model. 

The term $(\sigma\ \ w\ \ \varphi)$ represents the world representing $\sigma$ survives after projecting the model on $w$ and in that world $\varphi$ is satisfiable. 

The term $(\sigma\ \ w\ \ \checkmark)$ represents that the world represented by $\sigma$ survives under projection of $w$ of the model.

The term $(\sigma_1,\sigma_2)$ represents in the model, the worlds represented by $\sigma_1$ and $\sigma_2$ should be indistinguishable to the agent.

Now we define the inference rules of our tableau proof system. Here an inference rule looks like:
\infer{C_1 | C_2 | \ldots | C_n}{%
                        A
                        }.

Here each $C_i$ and $A$ is a set of tableau terms. The $C_i$s are called consequence, $A$ is the antecedent.

A tableau proof can be assumed a tree. Each node of the tree is a set of tableau terms $\Gamma$. An inference rule can be applied in the following way:

If $A\subseteq\Gamma$ and $C_i$'s are not in $\Gamma$, the children of $\Gamma$ are $\Gamma\union C_i$ for each $i\in[n]$.

When no rules can be applied on a $\Gamma$, we say $\Gamma$ is saturated (leaf node in the proof tree).

If $\bot\in\Gamma$, we say that branch is closed. If all branch of the proof tree is closed, we say the tableau is closed, else is open.

Given a $\POL_1$ formula $\varphi$, we start with $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma,\sigma), (\sigma\ \ \epsilon\ \ \checkmark)\}$.

\subsection{Rules}
% \begin{itemize}
%     \item Propositional Rules
%     \begin{itemize}
%         \item Clash rule:
%         \infer{\bot}{%
%                         (\sigma
%                         & w
%                         & p),
%                         & (\sigma
%                         & w
%                         & \neg p)
%                         }, $p\in\mathcal{P}$
%         \item Constant Valuation if:
%         \infer{(\sigma\ \ w\ \ [a]p)}{%
%                         (\sigma
%                         & w
%                         & p)
%                         }, $p\in\mathcal{P}$             
%         \item Constant Valuation Negation if:
%         \infer{(\sigma\ \ w\ \  [a]\neg p)}{%
%                         (\sigma
%                         & w
%                         & \neg p)
%                         }, $p\in\mathcal{P}$

%         \item AND rule:
%         \infer{(\sigma\ \ w\ \ \psi),(\sigma\ \ w\ \  \chi)}{%
%                         (\sigma
%                         & w
%                         & \psi\wedge\chi)
%                         }

%         \item OR rule:
%         \infer{(\sigma\ \ w\ \ \psi)\ \ |\ \ (\sigma\ \ w\ \ \chi)}{%
%                         (\sigma
%                         & w
%                         & \psi\vee\chi)
%                         }

        
%     \end{itemize}

%     \item Knowledge Rules
%     \begin{itemize}
%         \item Knowledge: 
%         \infer{(\sigma'\ \ w\ \ \psi)}{%
%                         (\sigma
%                         & w
%                         & K\psi),
%                         &(\sigma'
%                         & w
%                         & \checkmark),
%                         &(\sigma, \sigma')
%                         }

%         \item Possibility:
%         \infer{(\sigma,\sigma_n), (\sigma_n\ \ w\ \ \checkmark), (\sigma_n\ \ w\ \  \psi), (\sigma_n, \sigma_n)}{%
%                         (\sigma
%                         & w
%                         & \hat{K}\psi)
%                         },
%         \infer{(\sigma,\sigma')}{%
%                         (\sigma, \sigma''),
%                         & (\sigma'',\sigma')
%                         },
%         \infer{(\sigma,\sigma')}{%
%                         (\sigma', \sigma)
%                         }

%         % \item No Miracle ? (\textbf{UNDECIDED}): 
%         % \infer{\sigma\ \ [a]\hat{K}\psi\ \ w}{%
%         %                 \sigma
%         %                 & \hat{K}\langle a\rangle\psi
%         %                 & w
%         %                 }
%     \end{itemize}

%     \item Diamond and Box Rules:
%     \begin{itemize}
%         \item Diamond Decompose:
%         \infer{(\sigma\ \ w\ \ \langle \pi\rangle\langle \pi'\rangle\psi)}{%
%                         (\sigma
%                         & w
%                         & \langle \pi\pi'\rangle\psi)
%                         }

%         % \item Box Decompose:
%         % \infer{(\sigma\ \ w\ \ [a][\pi]\psi)}{%
%         %                 (\sigma
%         %                 & w
%         %                 & [a\pi]\psi)
%         %                 }
                        
%         \item Diamond ND Decompose:
%         \infer{(\sigma\ \ w\ \ \ldiaarg{\pi_1}\psi)\ \ |\ \ (\sigma\ \ w\ \ \ldiaarg{\pi_2}\psi)}{%
%                         (\sigma
%                         & w
%                         & \ldiaarg{\pi_1 + \pi_2}\psi)
%                         }

%         % \item Box ND Decompose:
%         % \infer{(\sigma\ \ w\ \ [\pi_1]\psi), (\sigma\ \ w\ \ \ [\pi_2]\psi)}{%
%         %                 (\sigma
%         %                 & w
%         %                 & [\pi_1 + \pi_2]\psi)
%         %                 }

%         \item Diamond Project: 
%         \infer{(\sigma\ \ wa\ \ \checkmark), (\sigma\ \ wa\ \ \psi)}{%
%                         (\sigma
%                         & w
%                         & \langle a\rangle\psi)
%                         }

%         \item Box Project:
%         \infer{(\sigma\ \ wa\ \ [\pi\regdiv a]\psi)}{%
%                         (\sigma
%                         & w
%                         & [\pi]\psi),
%                         & (\sigma\ \ wa\ \ \checkmark)
%                         }

%         \item Empty Box:
%         \infer{(\sigma\ \ w\ \ \psi)}{%
%                         (\sigma
%                         & w
%                         & [\epsilon]\psi)
%                         }
                        
%         \item Project Determinism:
%         \infer{(\sigma\ \ w\ \ [a]\psi)}{%
%                         (\sigma
%                         & w
%                         & \langle a\rangle\psi)
%                         }
                        
%         % \item Perfect Recall ? (\textbf{UNDECIDED}):
%         % \infer{\sigma\ \ \hat{K}\langle a\rangle\psi\ \ w}{%
%         %                 \sigma
%         %                 & \langle a\rangle\hat{K}\psi
%         %                 & w
%         %                 }
%     \end{itemize}
    
%     \item Survival Rules:
%     \begin{itemize}
%         \item Constant Valuation Up:
%         \infer{(\sigma\ \ \epsilon\ \ p)}{%
%                         (\sigma
%                         & w
%                         & p)
%                         },
%         \infer{(\sigma\ \ \epsilon\ \ \neg p)}{%
%                         (\sigma
%                         & w
%                         & \neg p)
%                         }, $p\in\mathcal{P}$
                        
%         \item Survival Chain:
%         \infer{(\sigma\ \ w\ \ \checkmark)}{%
%                         (\sigma
%                         & wa
%                         & \checkmark)
%                         }, $a\in\Sigma, w\in\Sigma^*$
%     \end{itemize}
% \end{itemize}

% \subsubsection{The Tableau Algorithm}
% Just like the single agent word case, here we propose an algorithm that creates the tableau tree $\mathcal{T}$ starting from the set of terms $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma, \sigma)\}$, given $\varphi$, as the root of $\mathcal{T}$.

% % \subsubsection{Proof that PR and NM Axiom Valid in $\POL_1$}
% % Here we prove two axioms, Perfect Recall ($\ldiaarg{a}\hat{K}\psi\rightarrow\hat{K}\ldiaarg{a}\psi$) and No Miracle($\hat{K}\ldiaarg{a}\psi\rightarrow[a]\hat{K}\psi$), to be valid in $\POL_1$.
% % \begin{theorem}
% % For any $\POL_1$ formula $\psi$, and any $\POL$ model $\M = \ldiaarg{W, R, V, Exp}$, $\M,s\vDash\ldiaarg{a}\hat{K}\psi\rightarrow\hat{K}\ldiaarg{a}\psi$.\label{theorem:PRvalidity}
% % \end{theorem}
% % \begin{proof}
% % Let us assume $\M,s\vDash\ldiaarg{a}\hat{K}\psi$.
% % \begin{align*}
% %     &\M,s\vDash\ldiaarg{a}\hat{K}\psi\\
% %     &\implies \M|_a,s\vDash\hat{K}\psi\\
% %     &\implies\exists(s,t)\in R_a\subseteq R\mbox{ and }\M|_a,t\vDash\psi\mbox{, where $R_a$ is the relation set of $\M|_a$}\\
% %     &\implies\M,t\vDash\ldiaarg{a}\psi\\
% %     &\implies\M,s\vDash\hat{K}\ldiaarg{a}\psi\mbox{, since $R_a\subseteq R$}
% % \end{align*}
% % \end{proof}
% % Next we prove validity of NM.
% % \begin{theorem}
% % For any $\POL_1$ formula $\psi$, and any $\POL$ model $\M = \ldiaarg{W, R, V, Exp}$, $\M,s\vDash\hat{K}\ldiaarg{a}\psi\rightarrow[a]\hat{K}\psi$.\label{theorem:NMvalidity}
% % \end{theorem}
% % \begin{proof}
% % Let us assume $\M,s\vDash\hat{K}\ldiaarg{a}\psi$.
% % \begin{align*}
% %     &\M,s\vDash\hat{K}\ldiaarg{a}\psi\\
% %     &\implies\exists(s,t)\in R\mbox{ and }\M,t\vDash\ldiaarg{a}\psi\\
% %     &\implies\M|_a,t\vDash\psi
% % \end{align*}
% % Now let us assume $s\notin W_a$ where $W_a$ is the set of worlds in $\M|_a$. Then vacuously, $\M,s\vDash[a]\hat{K}\psi$.

% % Now suppose $s\in W_a$. Hence $(s,t)\in R_a$, where $R_a\subseteq R$ is the set of indistinguishability relation of $\M|_a$. Therefore $\M|_a,s\vDash\hat{K}\psi$. This implies $\M,s\vDash[a]\hat{K}\psi$.
% % \end{proof}

% Given a formula $\varphi$:
% \begin{enumerate}
%     \item Let $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$

%     \item Let$\mathcal{T}$ be a tree of set of terms of tableau with $\Gamma$ in the root.
    
%     \item While there is a case matching from $(a)$ to $(c)$ and new terms can be inferred:
%     \begin{enumerate}
%         \item there is a leaf in $\mathcal{T}$ that has no $\bot$ term and it is not saturated against Propositional and Survival Rules then :
%         \begin{enumerate}
%             \item Let $\Gamma$ be the leaf.
%             \item Let $(\sigma\ \ w\ \ \psi)$ or $(\sigma\ \ w\ \ \checkmark)$ be the term that are unsaturated.
%             \item $\Gamma' = \Gamma$
%             \item If $\psi = l$ where $l$ is of the form either $p$ or $\neg p$, where $p$ is a propositional letter then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union \{(\sigma\ \ w\ \ [a]\psi), (\sigma\ \ \epsilon\ \ \psi)\}$, by Constant valuation if and Up
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
            
%             \item Else If $\psi = \psi_1\wedge\psi_2$ then 
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ \psi_1), (\sigma\ \ w\ \ \psi_2)\}$
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
        
%             \item Else If $\psi = \psi_1\vee\psi_2$ then 
%             \begin{enumerate}
%                 \item $\Gamma'_1 = \Gamma'\union\{(\sigma\ \ w\ \ \psi_1)\}$
                
%                 \item $\Gamma'_2 = \Gamma'\union\{(\sigma\ \ w\ \ \psi_2)\}$
                
%                 \item Add $\Gamma'_1$ and $\Gamma'_2$ as children of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
            
        
%             \item Else If $\{(\sigma\ \ w\ \ \psi), (\sigma\ \ w\ \ \neg\psi)\}\subseteq\Gamma$ then
%             \begin{enumerate}
%                 \item  $\Gamma' = \Gamma'\union\{\bot\}$
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
           
%             \item Else
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w'\ \ \checkmark)\mid w'\in Pre(\LL(w))\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
%         \end{enumerate}
        
%         \item Else If there is a leaf in $\mathcal{T}$ that has no $\bot$ term, is  saturated against Propositional and Survival Rules but not saturated against Knowledge Rules then 
%         \begin{enumerate}
%             \item Let the leaf be $\Gamma$ and $(\sigma\ \ w\ \ \psi)$ be a Knowledge unsaturated term.
            
%             \item $\Gamma' = \Gamma$
            
%             \item If $\psi = K\chi$ then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma'\ \ w\ \ \chi)\mid \{(\sigma,\sigma'), (\sigma'\ \ w\ \ \checkmark)\}\subseteq\Gamma\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
            
%             \item Else If $\psi = \hat{K}\chi$ then 
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma_n, \sigma_n), (\sigma_n\ \ w\ \ \checkmark), (\sigma_n\ \ w\ \ \chi)\}\union\{(\sigma', \sigma_n), (\sigma_n, \sigma')\mid (\sigma'\ \ w\ \ \checkmark)\in\Gamma\}$
                
%                 \item  Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
%         \end{enumerate}
%         \item Else if there is a leaf in $\mathcal{T}$ that has no $\bot$ term, is  saturated against Propositional, Survival Rules and Knowledge Rules, but not saturated against Diamond and Box Rules then
%         \begin{enumerate}
%             \item Let $\Gamma$ be the unsaturated leaf and $(\sigma\ \ w\ \ \psi)$ be the unsaturated term
            
%             \item $\Gamma' = \Gamma$
%             \item If $\psi = [\pi_1\pi_2]\chi$ then 
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ [\pi_1][\pi_2]\chi)\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
%             \end{enumerate}
%             \item Else If $\psi = \ldiaarg{\pi_1\pi_2}\chi$  then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ \ldiaarg{\pi_1}\ldiaarg{\pi_2}\chi)\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
%             \end{enumerate}
            
%             \item Else If $\psi = [\pi_1 + \pi_2]\chi$ then 
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ [\pi_1]\psi), (\sigma\ \ w\ \ [\pi_2]\psi)\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
%             \end{enumerate}
            
%             \item Else If $\psi = \ldiaarg{\pi_1 + \pi_2}\chi$ then
%              \begin{enumerate}
%                 \item $\Gamma_1 = \Gamma'\union\{(\sigma\ \ w\ \ \ldiaarg{\pi_1}\psi)\}$
                
%                 \item $\Gamma_2 = \Gamma'\union\{ (\sigma\ \ w\ \ \ldiaarg{\pi_2}\psi)\}$.
                
%                 \item Add $\Gamma_1$ and $\Gamma_2$ as children of $\Gamma$ in $\mathcal{T}$
%             \end{enumerate}
            
%             \item Else If $\psi = \ldiaarg{a}\chi$ then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ wa\ \ \chi), (\sigma\ \ wa\ \ \checkmark), (\sigma\ \ w\ \ [a]\chi)\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
%             \end{enumerate}
            
%             \item Else If $\psi = [a]\chi$ and $(\sigma\ \ wa\ \ \checkmark)\in\Gamma$ then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma\union\{(\sigma\ \ wa\ \ \chi)\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
%         \end{enumerate}
%     \end{enumerate}
    
%     \item Traverse through the leaves of $\mathcal{T}$.
%     \item If there is a leaf with no $\bot$ in it, return SAT, else UNSAT.
% \end{enumerate}





\subsubsection{Termination}
\begin{theorem}
Given the formula $\varphi$, the tableau proof for satisfiability terminates.
\label{lemma:terminationstartfreeone}
\end{theorem}
\begin{proof}
We can prove that a term like $(\sigma\ \ w\ \ \psi)$, for any $w$, any $\sigma$ and any $\psi\in FL(\varphi)$, the tableau proof for $\{(\sigma\ \ w\ \ \psi), (\sigma,\sigma), (\sigma\ \ w\ \ \checkmark)\}$ terminates, by induction on the size of $\psi$.

\textbf{Base Case.} Consider the case where $\psi = p$ where $p$ is a propositional letter. Starting from $\Gamma = \{(\sigma\ \ w\ \ \psi), (\sigma,\sigma), (\sigma\ \ w\ \ \checkmark)\}$, the tableau applies constant valuation rule once and then the tableau terminates here since no more rule can be applied.

\textbf{Induction Hypothesis.} Let the statement be true for any $\psi$ such that $|\psi| \leq n$.

\textbf{Induction Step.} Consider $\psi$ such that $|\psi| = n + 1$. We go case by case in syntax of $\psi$:
\begin{itemize}
    \item $\psi = \chi\wedge\xi$. Here, the AND rule gets applied to produce $(\sigma\ \ w\ \ \chi)$ and $(\sigma\ \ w\ \ \xi)$, and by IH proof for them terminates.
    
    \item $\psi = \chi\vee\xi$. Here the OR rule will give $(\sigma\ \ w\ \ \chi)$ or $(\sigma\ \ w\ \ \xi)$ which again is terminating.
    
    \item $\psi = K\chi$. By the knowledge rule , the term $(\sigma \ \ w\ \ \chi)$ will be added. (We start by $(\sigma,\sigma)$). By IH, this terminates.
    
    \item $\psi = \hat{K}\chi$. By the possibility rule, we introduce a new label $\sigma_n$ and term $(\sigma_n\ \ w\ \ \psi)$ along with additional relational terms. By IH, proof for this terminates.
    
    \item $\psi = \ldiaarg{\pi\pi'}\chi$. By the diamond decompose we derive $(\sigma\ \ w\ \ \ldiaarg{\pi}\ldiaarg{\pi'}\chi)$. By IH, the proof for this terms terminate. 
    
    \item $\psi = \ldiaarg{\pi_1 + \pi_2}\chi$. By the diamond ND decompose, we derive $(\sigma\ \ w\ \ \ldiaarg{\pi_1}\chi)$ or $(\sigma\ \ w\ \ \ldiaarg{\pi_2}\chi)$. By IH, the proof for them terminates. 
    
    \item $\psi = [\pi]\psi$. If $\pi\neq\epsilon$ and $(\sigma\ \ wa\ \ \checkmark)$, the rule derives $(\sigma\ \ wa\ \ [\pi\regdiv a])$. Hence by IH, the proof for this terminates. The other case where $\pi = \epsilon$ is trivial.
\end{itemize}

Now for every $\hat{K}$, there arrives a new label $\sigma'$, and for every $\ldiaarg{a}$ operator, a letter gets added in $w$. Hence $\#\sigma$ is finite, where $\#\sigma$ is number of unique world labels. Also since max legnth of such a $w$ is at most $O(|\varphi|)$, because of survival chain, there can be $|w|$ many terms derived and hence polynomial to size of $|\varphi|$ such terms. Since there can be at most $\Sigma^{|w|}$ such unique words, hence the proof terminates, that is arrives at a point where it cannot derive more new terms.
\end{proof}
% \begin{corollary}
% The Satisfiability problem of single agent star-free fragment of $\POL$ takes at most exponential steps to decide with respect to size of input formula $\varphi$. 
% \end{corollary}


\subsubsection{Soundness and Completeness}
\begin{theorem}
Given a formula $\varphi$, if $\varphi$ is satisfiable, then the tableau for $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$ is open.
\end{theorem}
\begin{proof}
We prove that if $\varphi$ is satisfiable then there exists a subtree rooted at some child $\Gamma_c$ of the root $\Gamma$ in $\mathcal{T}$ which is open using induction on the depth of the tableau tree $\mathcal{T}$. Let the pointed epistemic model that satisfy $\varphi$ be $\M,s$.

\textbf{Base Case.} Let the base case be $|\Gamma| = 2 + 1$. Since we start from $\{(\sigma\ \ \epsilon\ \ \varphi), (\sigma, \sigma), (\sigma\ \ \epsilon\ \ \checkmark)\}$. Hence this implies $\varphi = l$ or $\varphi = [a]\psi$, where $l$ is a literal (a positive propositional letter or a negation of it). Hence the tableau remains open since no $\bot\in\Gamma$.

\textbf{Induction Hypothesis.} Let the statement be true for any tableau tree $\mathcal{T}$ of depth at most $n$.

\textbf{Inductive Step.} Consider the tableau tree $\mathcal{T}$ rooted at $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma, \sigma), (\sigma\ \ \epsilon\ \ \checkmark)\}$ of depth at most $n + 1$. Now we go case by case with $\varphi$:
\begin{itemize}
    \item $\varphi = \psi\wedge\chi$: We apply AND rule, and hence $\Gamma' = \Gamma\union\{(\sigma\ \ \epsilon\ \ \psi), (\sigma\ \ \epsilon\ \ \chi)\}$, which is a child rooted at $\Gamma$. Since $\M,s\vDash\varphi$, by definition $\M,s\vDash\psi$ and $\M,s\vDash\chi$. By IH, tableau tree rooted at $\Gamma'$ is open, which suggestes, $\mathcal{T}$ is open.
    
    \item $\varphi = \psi\vee\chi$: We apply OR rule and hence we get two children, $\Gamma_1 = \Gamma\union\{(\sigma\ \ \epsilon\ \ \psi)\}$ and $\Gamma_2 = \Gamma\union\{(\sigma\ \ \epsilon\ \ \chi)\}$. Since $\M,s\vDash\psi\vee\chi$, hence $\M,s\vDash\psi$ or $\M,s\vDash\chi$. By IH, one of the sub tableau tree rooted at $\Gamma_1$ or $\Gamma_2$ will be open, hence implying $\mathcal{T}$ to be open.
    
    \item $\varphi = K\psi$: By applying the Knowledge rule, $\Gamma' = \Gamma\union\{(\sigma'\ \ \epsilon\ \ \psi)\mid \{(\sigma, \sigma'), (\sigma'\ \ \epsilon\ \ \checkmark)\}\subseteq\Gamma\}$. Since $\M,s\vDash K_i\psi$, hence for every $s'\in\M$ such that $s\sim s'$, $\M,s'\vDash\psi$. By IH, the tableau subtree rooted at $\Gamma'$ is open.
    
    \item $\varphi = \hat{K}\chi$: By applying the possibility rule, $\Gamma' = \Gamma\union\{(\sigma_n, \sigma_n), (\sigma_n\ \ \epsilon\ \ \checkmark), (\sigma_n\ \ \epsilon\ \ \chi)\}\union\{(\sigma, \sigma_n), (\sigma_n, \sigma)\}\union\{(\sigma', \sigma_n), (\sigma_n, \sigma')\mid \{(\sigma'\ \ \epsilon\ \ \checkmark), (\sigma,\sigma')\}\subseteq\Gamma_l\}$. Since, $\M,s\vDash\hat{K}\chi$, hence there is an $s_n\in\M$ such that $\M,s_n\vDash\chi$, also $s_n\sim s'$ for every $s'\in\M$ since $\sim$ is an equivalence relation. Hence by IH, the sub tableau tree rooted at $\Gamma'$ is open.

    \item $\varphi = \ldiaarg{\pi + \pi'}\psi$. Since $\M,s\vDash\ldiaarg{\pi + \pi'}\psi$, hence this implies, by truth definition, $\M,s\vDash\ldiaarg{\pi}\psi$ or $\M,s\vDash\ldiaarg{\pi'}\psi$. Hence by IH, one of sub tableau rooted at $\Gamma\union\{(\sigma\ \ \epsilon\ \ \ldiaarg{\pi}\psi)\}$ or $\Gamma\union\{\sigma\ \ \epsilon\ \ \ldiaarg{\pi'}\psi\}$ is open. 
    
    \item $\varphi = \ldiaarg{\pi\pi'}\psi$:  Hence by the diamond decomposition rule $\Gamma' = \Gamma\union\{(\sigma\ \ \epsilon\ \ \ldiaarg{\pi}\ldiaarg{\pi'}\psi)\}$. Since $\M,s\vDash\ldiaarg{\pi\pi'}\psi$, hence $\M|_{w_*},s\vDash\psi$, for some $w_*\in\LL(\pi\pi')$ which also suggests, there is a $w\in\LL(\pi)$ and a $w'\in\LL(\pi')$ such that $w_* = ww'$. Hence   $\M|_w,s\vDash\ldiaarg{\pi'}\psi$, which implies $\M,s\vDash\ldiaarg{\pi}\ldiaarg{\pi'}\psi$. By IH, the tableau for $\Gamma'$ is open.
    
    
    \item $\varphi = \ldiaarg{a}\psi$. Hence now by Projection rule, $\Gamma' = \Gamma\union\{(\sigma\ \ a\ \ \checkmark), (\sigma\ \ a\ \ \psi)\}$. Since $\M,s\vDash\ldiaarg{a}\psi$, therefore $s\in\M|_a$ and $\M|_a,s\vDash\psi$. And hence by IH, tableau tree rooted at $\Gamma'$ is open. 

    \item $\varphi = [\pi]\psi$. Say $(\sigma\ \ a\ \ \checkmark)$ is added for some diamond formula term, say of the form $(\sigma\ \ \epsilon\ \ \ldiaarg{a}\psi')$, hence the proof has added $(\sigma\ \ a\ \ [\pi\regdiv]\psi)$. By assumption $\M, s\vDash\ldiaarg{a}\psi'$, and hence $s\in\M|_a$. Therefore $\M|_a,s\vDash[\pi\regdiv a]\psi$, hence the proof starting from terms $\{(\sigma, \sigma), (\sigma\ \ a\ \ \checkmark), (\sigma\ \ a\ \ [\pi\regdiv a]\psi)\}$ will remain open.

    For the other case $(\sigma\ \ a\ \ \checkmark)$ is not added, hence $s\notin\M|_a$, therefore the tableau remains open.
\end{itemize}
\end{proof}

\begin{theorem}
Given a formula $\varphi$, if the tableau for $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$ is open, then $\varphi$ is satisfiable.\label{theorem:starfreeonecomplete}
\end{theorem}
\begin{proof}
Since by assumption, the tableau for $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$ is open, there exists a branch in the tableau tree where in the leaf node there is  a set of terms $\Gamma_l$ such that it is saturated and $\bot\notin\Gamma_l$.

Now we create a model $\M = \ldiaarg{W, R, V, Exp}$ out of $\Gamma_l$ and prove that $\varphi$ is satisfied by some world in the model.

\begin{itemize}
    \item $W = \{s_\sigma\mid \sigma\mbox{ is a distinct label in the terms occuring in }\Gamma_l\}$
    
    \item $R = \{\{s_{\sigma_1}, s_{\sigma_2}\}\mid(\sigma_1,\sigma_2)\in\Gamma_l\}$
    
    \item $V(s_\sigma) = \{p\mid (\sigma\ \ \epsilon\ \ p)\in\Gamma_l\}$
    
    \item $Exp(s_\sigma) = \sum_{w\in\Lambda}w$, where $\Lambda = \{w\mid (\sigma\ \ w\ \ \checkmark)\in\Gamma_l\mbox{ and }\nexists w':((\sigma\ \ w'\ \ \checkmark)\in\Gamma_l\mbox{ and }w\in \LL(Pre(w')))\}$
\end{itemize}

Note that, new world label $\sigma_n$ is only created in the possibility rule, with a reflexive relation on itself. Now cosider the set $R' = \{(\sigma, \sigma')\mid \{(sigma\ \ w\ \ \checkmark), (\sigma' \ \ w'\ \ \checkmark)\}\subseteq\Gamma_l\}$. Hence this can be considered a binary relation over the set of all distinct $\sigma$ that occurs in $\Gamma_l$. When a $\sigma'$ is created by possibility rule, it is refexive. Also by the relation rules in possibility rule, they are made symmetrically related with every other label that has been previously there. Hence $R'$ is an equivalence relation, hence making $R$ in the model an equivalence relation.


Now we shall prove the following two statement:

\textbf{If $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$ then $s_{\sigma}$ survives in $\M|_w$}

and 

\textbf{For any word $w$ that occurs in $\Gamma_l$, any label $\sigma$ and any formula $\psi$, If $(\sigma\ \ w\ \ \psi)\in\Gamma_l$ and $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$ then $s_{\sigma}$ survives in $\M|_w$ and  $\M|_w,s_\sigma\vDash\psi$}.



For the first statement, we induct on the size of $|w|$.

\textbf{Base Case.} Let $|w| = 1$. Hence $w \in \{\epsilon\}\union \Sigma$ . Since $\Gamma\subseteq\Gamma_l$ and $(\sigma\ \ \epsilon\ \ \checkmark)$, and $w_\sigma$ is in $\M|_\epsilon = \M$.

For the case $w = a$ for any $a\in\Sigma$. Hence there exists a word $w'$ that occurs in a term in $\Gamma_l$ labelled by $\sigma$ such that $w\in\LL(Pre(w'))$ and there is no other word bigger than $w'$ such that $w'$ is in its prefix. Hence by definition of $w'\in\LL(Exp(s_\sigma))$ which guarantees survival of $s_\sigma$ in $\M|_a$. 

\textbf{Induction Hypothesis.} Assume the statement to be true for $|w| = n$.

\textbf{Inductive Step.} Consider the case where $|w| = n + 1$. 

By assumption, $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$. Hence by the fact that $\Gamma_l$ is saturation and by rule "Survival Chain", there is $(\sigma\ \ w'\ \ \checkmark)\in\Gamma_l$, where $w = w'a$ for some $a\in\Sigma$. Hence by IH, the result follows that $s_\sigma$ survives in $\M|_{w'}$. 

Now, since $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$, there is a $w''$ occurring in a term of form $(\sigma\ \ w''\ \ \checkmark)\in\Gamma_l$  such that $w\in \LL(Pre(w''))$ and there is no $w'''$ such that $(\sigma\ \ w'''\ \ \checkmark)\in\Gamma_l$ and $w''\in\LL(Pre(w'''))$. Hence, by definition of the model ($Exp$), $w''\in\Lambda$, which further suggests $w''\in\LL(Exp(s_\sigma))$. Since $w\in\LL(Pre(w''))$ and $s_\sigma$ is in $\M|_{w'}$, therefore $s_\sigma$ survives in $\M|_{w}$. This proves the first part of the proof that if $(\sigma\ \ w\ \ \checkmark)\in\Gamma_l$, then $s_\sigma$ survives in $\M|_w$.

\textbf{Proof for Second Statement.}
Naturally, we shall induct upon the size of $\psi$. 

\textbf{Base Case.} Let $\psi$ is of the form $p$ or $\neg p$. By the definition of the function $V$ for the model and the previous proof, the statement stands true.

\textbf{Induction Hypothesis.} Let us consider the statement is true for any $\psi$ such that $|\psi|<n'$ for some $n'$.

\textbf{Inductive Step.} We prove for $|\psi| = n'$. Again, we go case by case on syntax of $\psi$. 
\begin{itemize}
    \item $\psi = \hat{K}\chi$. Since $\Gamma_l$ is saturated, by the rule of possibility, $\{(\sigma'\ \ w\ \ \chi), (\sigma, \sigma'), (\sigma'\ \ w\ \ \checkmark)\}\subseteq\Gamma_l$. By IH on the subformula $\chi$, definition of model, the proof of previous statement, and the rule "survival chain", $s_{\sigma'}$ survives in $\M|_{w}$ and $\M|_w,s_{\sigma'}\vDash\chi$. Also by definition, $\{s_{\sigma}, s_{\sigma'}\}\in R$, hence proving $\M|_w, s_\sigma\vDash\hat{K}\chi$.
    
    \item $\psi = K\chi$. Since $\Gamma_l$ is saturated, and by previous statement $s_{\sigma'}$ is surviving for every $(\sigma'\ \ w\ \ \checkmark)$, by the rule of knowledge $(\sigma'\ \ w\ \ \chi)\in\Gamma_l$ for every $(\sigma, \sigma')$. Hence by IH on subformula, $\M|_w, s_{\sigma'}\vDash\chi$ for every $\sigma'$ such that $\{\sigma,\sigma'\}\in R$.

    \item $\psi = \ldiaarg{\pi + \pi'}\chi$. Since $\Gamma_l$ is saturated, hence by the ND Decomposition, either the term $(\sigma\ \ w\ \ \ldiaarg{\pi}\chi)\in\Gamma_l$ or $(\sigma\ \ w\ \ \ldiaarg{\pi'}\chi)\in\Gamma_l$. By IH, $\M|_w,s_\sigma\vDash\ldiaarg{\pi}\chi$ or $\M|_w,s_\sigma\vDash\ldiaarg{\pi'}\chi$ and hence $\M|_w,s_\sigma\vDash\ldiaarg{\pi + \pi'}\chi$.

    \item $\psi = \ldiaarg{\pi\pi'}\chi$. Since $\Gamma_l$ is saturated, hence $(\sigma\ \ w\ \ \ldiaarg{\pi}\ldiaarg{\pi'}\chi)\in \Gamma_l$. By IH, since $\ldiaarg{\pi}\ldiaarg{\pi'}\chi\in FL(\psi)$, hence $\M|_w, s_\sigma\vDash\psi$.
    
    \item $\psi = \ldiaarg{a}\chi$. Note that we dont consider a general word $w'$ in the diamond as given $w' = aw''$, a formula $\ldiaarg{w'}\chi$ is satisfiable if and only if $\ldiaarg{a}\ldiaarg{w''}\chi$ is satisfiable.

    \item $\psi = [\pi]\chi$. Let us consider $(\sigma\ \ wa\ \ \checkmark)\in\Gamma_l$ for some $a\in\Sigma$. Hence by the proof of first statement, $s_\sigma\in\M|_{wa}$. Also $|\LL(\pi)| < |\LL(\pi\regdiv a)|$. Hence by induction on the size of formula $\M|_{wa},s\sigma\vDash[\pi\regdiv a]\chi$ which implies $\M|_w,s_\sigma\vDash[\pi]\chi$. 

    % Since $\Gamma_l$ is saturated, by projection rule, there is  $\{(\sigma\ \ wa\ \ \checkmark), (\sigma\ \ wa\ \ \chi)\}\subseteq \Gamma_l$. By previous statement, therefore $s_\sigma$ survives in $\M|_{wa}$, and by IH, $\M|_{wa}, s_\sigma\vDash\chi$. Hence $\M|_w, s_\sigma\vDash\ldiaarg{a}\chi$. The box proof goes similarly.
\end{itemize}
\end{proof}

\subsubsection{An NPSPACE Algorithm}
In this section we prove that deciding whether a Starfree Single agent POL formula is satisfiable uses polynomial space with respect to the input formula.

\begin{theorem}
A formula $\varphi$ is Starfree $\POL_1$ satisfiable iff it can satisfied by a model of at most $O(|\varphi|)$ worlds, each having expectation of size at most $O(p(|\varphi|))$, where $p(X)$ is some polynomial in $X$.
\label{theorem:starfreeonesmall}
\end{theorem}
\begin{proof}
Assuming there is a model of at most $O(|\varphi|)$ worlds, proving $\varphi$ is satisfiable is trivial.

We prove the converse. We assume that $\varphi$ is satisfiable. Since it is satisfiable, we can build a model $\M$ from its open tableau just like we created in proof of theorem \ref{theorem:starfreeonecomplete}. Consider the $\M = \ldiaarg{W, R, V, Exp}$ and say $\M,s\vDash\varphi$. Note that, $\varphi$ is in negation normal form. First we partition the set $W$ using the following equivalence relation $\equiv$:
\begin{itemize}
    \item $s\equiv s$.
    \item $s'\equiv s''$, for every $s',s''\neq s$, iff for $\hat{K}\psi\in FL(\varphi)$, $\M,s'\vDash\psi$ and $\M,s''\vDash\psi$
\end{itemize}

Let us denote the partition by $\equiv$ as $s_\varphi = [s]_\equiv$, where $\M,s\vDash\varphi$ and $s_\psi = [s']_\equiv$ where for any $s'\in [s']_\equiv$, there is some $\hat{K}\psi\in FL(\varphi)$ such that $\M,s'\vDash\psi$.

Now we create a model $\M' = \{W', R', V', Exp'\}$ as following:
\begin{itemize}
    \item $W' = \{s_\varphi\}\union \{s_\psi\mid \hat{K}\psi\in FL(\varphi)\}$.
    \item $R' = \{(s_\psi,s_{\psi'})\mid s_\psi\in W', s_{\psi'}\in W'\}$
    \item $V'(s_\psi) = V(s')$ where $s'\in s_\psi$.
    \item $Exp'(s_\varphi) = Exp(s)$.
    
    $Exp'(s_\psi) = \sum_{s'\in s_\psi} Exp(s')$.
\end{itemize}


Now we shall prove for any $w\in\Sigma^*$ occuring in tableau of $\varphi$, for any $\psi\in FL(\varphi)$, for any $s'\in W'$
\begin{align*}
    \exists s''\in s' &\M|_w,s''\vDash\psi\\
                    &\mbox{ iff }\\
                    \M'|_w,&s'\vDash\psi
\end{align*}
We induct on the size of $\psi$.

\textbf{Base Case.} The case of $\psi = p$ or $\psi = \neg p$, where $p$ is a propositional letter. By definition of $V'$ in the definition of $\M'$, the result holds.

\textbf{Induction Hypothesis.} Let the statement be true for any $\psi$ of size at most $n$.

\textbf{Inductive Step.} Consider $\psi$ such that $|\psi| = n + 1$.
\begin{itemize}
    \item $\psi = \hat{K}\chi$. Assume there is a $s_1\in s'$ such that $\M|_w,s_1\vDash\hat{K}\chi$, which implies there is a $t\in W$ such that $\M|_w,t\vDash\chi$. 
    
    Now $\hat{K}\chi\in FL(\varphi)$, and since the $\M$ is complete (every world is related to every other world), $\M|_w,s\vDash\hat{K}\chi$, where $s\in s_\varphi$ (since $\varphi$ is assumed satisfiable, hence $s$ is surviving in $\M|_w$). Therefore, by the partition definition (definition of the equivalence relation), there is a partition $s_\chi$ such that $t\in s_\chi$.
    
    By IH, $\M'|_w, s_\chi\vDash$ and hence $\M'|_w,s'\vDash\hat{K}\chi$.
    
    Conversely, let $\M'|_w, s'\vDash\hat{K}\chi$. Hence there is a $t'\in W'$ where $\M'|_w,t'\vDash\chi$. By IH, there is a $t\in t'$ such that $\M|_w,t\vDash\chi$. Since $\M$ is a complete model, $\M|_w,s\vDash\hat{K}\psi$.
    
    Similarly can be proven for $\psi = K\chi$.
    
    \item $\psi = \ldiaarg{a}\chi$. 
    Let us assume $\M|_w, s_1\vDash\ldiaarg{a}\chi$ for some $s_1\in s'$. Now two cases are possible, $s' = s_\varphi$, which implies $s_1 = s$. By assumption, $\M|_{wa}, s_1\vDash\chi$. By definition, $Exp'(s_\varphi) = Exp(s_1)$. Hence, since $s_1$ is surviving after projection on $wa$, $s_\varphi$ shall also survive after projection on $wa$. By IH, $\M'|_{wa}, s_\varphi\vDash\chi$, which implies $\M'|_w,s_\varphi\vDash\ldiaarg{a}\chi$.
    
    Another case that is possible is $s'\neq s_\varphi$. In that case, by the definition of $Exp'(s')$, $\LL(Exp(s_1))\subseteq \LL(Exp(s'))$. Hence in this case too, $s'$ survives the projection on $wa$. And hence, similarly by IH, our statement holds true.
    
    Conversely, let $\M'|_w, s'\vDash\ldiaarg{a}\chi$. Note that, by definition of the Expectation function, $\LL(Exp'(s')) = \bigcup_{s_0\in s'}\LL(Exp(s_0))$. By assumption $\M'|_{wa},s'\vDash\chi$. By the definition of Expectation function, there exists some $w'\in\bigcup_{s_0\in s'}\LL(Exp(s_0))$ for which $s'$ survives the projection on $wa$, that is $wa\in\LL(Pre(w'))$. Therefore there is some world $s_1\in s'$, which survives the projection and by IH, $\M|_{wa}, s_1\vDash\chi$, which gives us the required result.
    
    Similarly can be proven for Box modality.
\end{itemize}

Also in the model $\M'$ we created, each world $s_\psi$ has Expectation such that $w\in\LL(Exp'(s_\psi))$ means $w$ has occurred in some term of the form $(\sigma\ \ w\ \ \checkmark)$ in the tableau proof for satisfiability. The size of such $w$ is at most $|\varphi|$ since $w$ gains one letter that $\varphi$ loses from its diamond operator. Also number of such maximal $w$'s (there is no $w'$ which has $w$ as prefix) will also be at most $|\varphi|$. Hence $|Exp'(s_\psi)|\leq O(q(|\varphi|))$ for some polynomial $q$.
\end{proof}
\begin{theorem}
    Deciding satisfiability of Single Agent Starfree Fragment can be done in polynomial space.
\end{theorem}
\begin{proof}
    The proof implies from theorem \ref{theorem:starfreeonesmall}. Since the model satisfying the input formula $\varphi$ can be of size polynomial with respect to $\varphi$, guessing such a model can be an $\NP$ procedure. 
    Verifying whether the model is satisfying the formula using polynomial space with respect to the size of $\varphi$ and the model, which again is polynomial size of $\varphi$.
\end{proof}



% Given a formula $\varphi$:
% \begin{enumerate}
%     \item Let $\Gamma = \{(\sigma\ \ \epsilon\ \ \varphi), (\sigma\ \ \epsilon\ \ \checkmark), (\sigma,\sigma)\}$

%     \item Let$\mathcal{T}$ be a tree of set of terms of tableau with $\Gamma$ in the root.
    
%     \item While there is a case matching from $(a)$ to $(c)$ and new terms can be inferred:
%     \begin{enumerate}
%         \item there is a leaf in $\mathcal{T}$ that has no $\bot$ term and it is not saturated against Propositional and Survival Rules then :
%         \begin{enumerate}
%             \item Let $\Gamma$ be the leaf.
%             \item Let $(\sigma\ \ w\ \ \psi)$ or $(\sigma\ \ w\ \ \checkmark)$ be the term that are unsaturated.
%             \item $\Gamma' = \Gamma$
%             \item If $\psi = l$ where $l$ is of the form either $p$ or $\neg p$, where $p$ is a propositional letter then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union \{(\sigma\ \ w\ \ [a]\psi), (\sigma\ \ \epsilon\ \ \psi)\}$, by Constant valuation if and Up
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
            
%             \item Else If $\psi = \psi_1\wedge\psi_2$ then 
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ \psi_1), (\sigma\ \ w\ \ \psi_2)\}$
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
        
%             \item Else If $\psi = \psi_1\vee\psi_2$ then 
%             \begin{enumerate}
%                 \item $\Gamma'_1 = \Gamma'\union\{(\sigma\ \ w\ \ \psi_1)\}$
                
%                 \item $\Gamma'_2 = \Gamma'\union\{(\sigma\ \ w\ \ \psi_2)\}$
                
%                 \item Non-deterministically choose among $\Gamma_1$ and $\Gamma_2$ and make it a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
            
        
%             \item Else If $\{(\sigma\ \ w\ \ \psi), (\sigma\ \ w\ \ \neg\psi)\}\subseteq\Gamma$ then
%             \begin{enumerate}
%                 \item  $\Gamma' = \Gamma'\union\{\bot\}$
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
           
%             \item Else
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w'\ \ \checkmark)\mid w'\in Pre(\LL(w))\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
%         \end{enumerate}
        
%         \item Else If there is a leaf in $\mathcal{T}$ that has no $\bot$ term, is  saturated against Propositional and Survival Rules but not saturated against Knowledge Rules then 
%         \begin{enumerate}
%             \item Let the leaf be $\Gamma$ and $(\sigma\ \ w\ \ \psi)$ be a Knowledge unsaturated term.
            
%             \item $\Gamma' = \Gamma$
            
%             \item If $\psi = K\chi$ then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma'\ \ w\ \ \chi)\mid \{(\sigma,\sigma'), (\sigma'\ \ w\ \ \checkmark)\}\subseteq\Gamma\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
            
%             \item Else If $\psi = \hat{K}\chi$ then 
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma_n, \sigma_n), (\sigma_n\ \ w\ \ \checkmark), (\sigma_n\ \ w\ \ \chi)\}\union\{(\sigma', \sigma_n), (\sigma_n, \sigma')\mid (\sigma'\ \ w\ \ \checkmark)\in\Gamma\}$
                
%                 \item  Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
%         \end{enumerate}
%         \item Else if there is a leaf in $\mathcal{T}$ that has no $\bot$ term, is  saturated against Propositional, Survival Rules and Knowledge Rules, but not saturated against Diamond and Box Rules then
%         \begin{enumerate}
%             \item Let $\Gamma$ be the unsaturated leaf and $(\sigma\ \ w\ \ \psi)$ be the unsaturated term
            
%             \item $\Gamma' = \Gamma$
%             % \item If $\psi = [\pi_1\pi_2]\chi$ then 
%             % \begin{enumerate}
%             %     \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ [\pi_1][\pi_2]\chi)\}$
                
%             %     \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
%             % \end{enumerate}
%             \item If $\psi = \ldiaarg{\pi_1\pi_2}\chi$  then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ \ldiaarg{\pi_1}\ldiaarg{\pi_2}\chi)\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
%             \end{enumerate}
            
%             % \item Else If $\psi = [\pi_1 + \pi_2]\chi$ then 
%             % \begin{enumerate}
%             %     \item $\Gamma' = \Gamma'\union\{(\sigma\ \ w\ \ [\pi_1]\psi), (\sigma\ \ w\ \ [\pi_2]\psi)\}$
                
%             %     \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
%             % \end{enumerate}
            
%             \item Else If $\psi = \ldiaarg{\pi_1 + \pi_2}\chi$ then
%              \begin{enumerate}
%                 \item $\Gamma_1 = \Gamma'\union\{(\sigma\ \ w\ \ \ldiaarg{\pi_1}\psi)\}$
                
%                 \item $\Gamma_2 = \Gamma'\union\{ (\sigma\ \ w\ \ \ldiaarg{\pi_2}\psi)\}$.
                
%                 \item Nondeterministically choose among $\Gamma_1$ and $\Gamma_2$ and make one of then child of $\Gamma$.
%             \end{enumerate}
            
%             \item Else If $\psi = \ldiaarg{a}\chi$ then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma'\union\{(\sigma\ \ wa\ \ \chi), (\sigma\ \ wa\ \ \checkmark), (\sigma\ \ w\ \ [a]\chi)\}$.
                
%                 \item For every term $(\sigma\ \ w\ \ [\pi]\chi_b)$:
%                 \begin{itemize}
%                     \item Build NFA $N_\pi = \ldiaarg{Q, \Sigma, q_0, \delta, F}$ of $\pi$. 
                    
%                     \item Create NFA $N'_{\pi} = \ldiaarg{Q\union\{q'_0\}, \Sigma, q'_0, \delta', F}$, where $\delta'(q,l) = \delta(q,l)$ for every $q\in Q, l\in\Sigma$ and $\delta'(q'_0, \epsilon) = \delta(q_0, a)$.
                    
%                     \item Create $\pi'$ which is a regular expression of $N'_\pi$.
                    
%                     \item $\Gamma' = \Gamma'\union\{(\sigma\ \ wa\ \ [\pi']\chi_b)\}$
%                 \end{itemize}
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$
%             \end{enumerate}
            
%             \item Else If $\psi = [a]\chi$ and $(\sigma\ \ wa\ \ \checkmark)\in\Gamma$ then
%             \begin{enumerate}
%                 \item $\Gamma' = \Gamma\union\{(\sigma\ \ wa\ \ \chi)\}$
                
%                 \item Add $\Gamma'$ as a child of $\Gamma$ in $\mathcal{T}$.
%             \end{enumerate}
%         \end{enumerate}
%     \end{enumerate}
    
%     \item Traverse through the leaves of $\mathcal{T}$.
%     \item If there is a leaf with no $\bot$ in it, return SAT, else UNSAT.
% \end{enumerate}


% \begin{breakablealgorithm}
% \caption{StarFree-SAT}
% \begin{algorithmic}[1]
% \Procedure{StarFree-SAT}{$\varphi$}
%     \State $T_{\sigma_0} \gets  \{(\epsilon, \varphi), (\epsilon, \checkmark)\}$ 
%     \State $T_{\sigma_0}$ is the root of tree $\cT_P$.
%     \While{there is a leaf of $\cT_P$ that satisfies one of the following conditions}
%         \If{$\bot\notin T_\sigma$ and $T_\sigma$ is unsaturated against Propositional and Survival Rules then}
%             \State Let $(w, \psi)$ or $(w, \checkmark)$ be the reason for unsaturation against the above rules.
            
%             \If{$\psi = \psi_1\wedge\psi_2$} $T_\sigma = T_\sigma\union\{(w, \psi_1),(w, \psi_2)\}$
            
%             \ElsIf{$\psi = \psi_1\vee\psi_2$} non deterministically choose $\psi_1$ or $\psi_2$ and $T_{\sigma} = T_\sigma\union\{(w, \psi_1)\}$ or $T_{\sigma} = T_\sigma\union\{(w, \psi_2)\}$ as per choice.
            
%             \ElsIf{$\psi = l$ where $l$ is a literal} $T_\sigma = T_\sigma\union\{(w, [a]l), (\epsilon, l)\}$.

%             \ElsIf{$\{(w, \psi), (w, \neg\psi)\}\subseteq T_\sigma$} $T_\sigma = T_\sigma\union\{\bot\}$.

%             \ElsIf{$(w, \checkmark)\in T_\sigma$} $T_\sigma = T_\sigma\union\{(w',\checkmark)\mid w'\in Pre(\LL(w))\}$.

%             \EndIf

%         \ElsIf{$\bot\notin T_\sigma$ and $T_\sigma$ is propositionally saturated but unsaturated against Box and Diamond Rules}
%             \State Let the reason for unsaturation be $(w, \psi)$.

%             \State If $\psi = \ldiaarg{\pi_1\pi_2}\psi'$ then $T_\sigma = T_\sigma\union\{(w,\ldiaarg{\pi_1}\ldiaarg{\pi_2}\psi')\}$.

%             \State If $\psi = \ldiaarg{\pi_1 + \pi_2}\psi'$ then nondeterministically choose a $\pi_i$, where $i\in\{1,2\}$ and make $T_\sigma = T_\sigma\union\{(w, \ldiaarg{\pi_i}\psi')\}$

%             \State If $\psi = \ldiaarg{a}\psi'$ then $T_\sigma = T_\sigma\union\{(wa, \checkmark), (wa, \psi'), (w, [a]\psi')\}$.

%             \State If $\psi = [\pi]\psi'$ and $(wa,\checkmark)\in T_\sigma$ then $T_\sigma = T_\sigma\union\{(wa, [\pi\regdiv a]\psi')\}$

%         \ElsIf{$\bot\notin T_\sigma$ and it saturated against Propositional, Survival and Box, Diamond Rules but for all formula $\psi$ that occurs in terms $(w, \psi)\in T_\sigma$, there is a $\psi'\in FL(\psi)$ such that neither $\psi'$ nor $\neg\psi'$ occurs in $T_\sigma$}
%             \State Non-deterministically choose $\psi'$ or $\neg\psi'$ and $T_\sigma = T_\sigma\union\{(w,\psi')\}$ or $T_\sigma = T_\sigma\union\{(w,\neg\psi')\}$ as per choice, where $\neg\psi'$ is in Negation normal form.

%         \ElsIf{$\bot\notin T_\sigma$ and $T_\sigma$ is saturated against Propositional rules, Survival Rules and Diamond, Box rules and there is no formula $\psi$ that occurs as $(w, \psi)\in T_\sigma$, there is a $\psi'\in FL(\psi)$ such that neither $\psi'$ nor $\neg\psi'$ occurs in $T_\sigma$}
%             \ForEach{$(w, \hat{K_i}\psi)\in T_\sigma$} 
%                 \State $T = \{(w, \hat{K_i}\psi')\mid (w, \hat{K_i}\psi')\in T_\sigma\}\union \{(w, K_i\psi')\mid (w, K_i\psi')\in T_\sigma\}\union\{(w, \psi)\}$
%                 \State If there is no $i$-ancestor $T_{\sigma''}$ of $T_\sigma$ such that $T\subseteq T_{\sigma''}$ then add a $i$-child $T_{\sigma'} = T$
%             \EndFor
%         \EndIf
%     \EndWhile
%     \While{$T_{\sigma_0}$ is not marked}
%         \If{there is an unmarked leaf node $T_\sigma$ of $\cT_P$}
%             \If{$\bot\in T_\sigma$ or $\{(w, K_i\psi), (w, \neg\psi)\}\subseteq T_\sigma$}
%                 \State Mark $T_{\sigma_0}$ "UNSAT"
%             \Else
%                 \State Mark $T_{\sigma_0}$ "SAT"
%             \EndIf

%         \Else
%             \State $T_\sigma$ is an unmarked internal node whose all children are marked.
%             \If{ all children of $T_\sigma$ is marked "SAT"}
%                 \State Mark $T_\sigma$ "SAT"
%             \Else
%                 \State Mark $T_\sigma$ "UNSAT"
%             \EndIf
%         \EndIf
%     \EndWhile
%     \If{$T_{\sigma_0}$ is marked "SAT"}
%         \State Return SAT
%     \Else 
%         \State Return UNSAT
%     \EndIf
%     \EndProcedure
% \end{algorithmic}
% \end{breakablealgorithm}

